A Categorical Framework for Modeling with Stock and Flow Diagrams

Stock and flow diagrams are already an important tool in epidemiology, but category theory lets us go further and treat these diagrams as mathematical entities in their own right. In this chapter we use communicable disease models created with our software, StockFlow.jl, to explain the benefits of the categorical approach. We first explain the category of stock-flow diagrams and note the clear separation between the syntax of these diagrams and their semantics, demonstrating three examples of semantics already implemented in the software: ODEs, causal loop diagrams, and system structure diagrams. We then turn to two methods for building large stock-flow diagrams from smaller ones in a modular fashion: composition and stratification. Finally, we introduce the open-source ModelCollab software for diagram-based collaborative modeling. The graphical user interface of this web-based software lets modelers take advantage of the ideas discussed here without any knowledge of their categorical foundations.

==> backup/preamble_copy.tex <==
\usepackage{amssymb,mathrsfs,amsmath,amsfonts,amsthm,graphicx,pdfpages,todonotes,bbold,float}
\usepackage{caption}
\usepackage{subcaption}

% Julia code
%\usepackage{minted}

% Quiver
%\usepackage{quiver}


% colors
\usepackage{xcolor}
\usepackage{framed,color}

\definecolor{shadecolor}{rgb}{1,0.8,0.3}
\definecolor{myurlcolor}{rgb}{0.5,0,0}
\definecolor{mycitecolor}{rgb}{0,0,0.7}
\definecolor{myrefcolor}{rgb}{0,0,0.7}
\definecolor{hyperrefcolor}{rgb}{0.5,0,0}

% hyperlinks

\usepackage{hyperref}
\hypersetup{
	colorlinks,
	linkcolor={hyperrefcolor},
	citecolor={mycitecolor},
	urlcolor={hyperrefcolor}
}


%\usepackage[clean]{svg}

% font for definitions 

\newcommand{\define}[1]{{\bf \boldmath{#1}}}

% call proofs "proof sketch"

\renewcommand*{\proofname}{Proof Sketch}

% sets

\newcommand{\namedset}[1]{\mathbb{#1}}
\newcommand{\N}{\namedset{N}}
\newcommand{\R}{\namedset{R}}
\newcommand{\Naturals}{\namedset{N}}
\newcommand{\Integers}{\namedset{Z}}

% categories

\newcommand{\namedcat}[1]{\mathsf{#1}}
\newcommand{\Set}{\namedcat{Set}}
\newcommand{\Fin}{\namedcat{Fin}}
\newcommand{\Graph}{\namedcat{Graph}}
\newcommand{\C}{\namedcat{C}}
\newcommand{\G}{\namedcat{G}}
\renewcommand{\H}{\namedcat{H}}
\newcommand{\K}{\namedcat{K}}
\newcommand{\Cat}{\namedcat{Cat}}
\newcommand{\CMC}{\namedcat{CMC}}
\newcommand{\CMon}{\namedcat{CMon}}
\newcommand{\Petri}{\namedcat{Petri}}
\newcommand{\cPetri}{\namedcat{cPetri}}
\newcommand{\Dynam}{\namedcat{Dynam}}
\newcommand{\StockFlow}{\namedcat{StockFlow}}
\newcommand{\Open}{\namedcat{Open}}

\newcommand{\4}{\mathbf{4}}
\newcommand{\8}{\mathbf{8}}

\newcommand{\X}{\namedcat{X}}
\newcommand{\A}{\namedcat{A}}

\newcommand{\id}[1]{\mathbb{1}_{#1}}
\newcommand{\compose}{\circ}
\newcommand{\dialspan}{\namedcat{DialSpan}(\namedcat{B},\namedcat{C})}
\newcommand{\product}{\&}
\newcommand{\coproduct}{\oplus}
\newcommand{\productmap}[2]{\langle #1, #2 \rangle}
\newcommand{\coproductmap}[2]{[#1,#2]}
\newcommand{\tensor}{\oslash}

\newcommand{\PSet}{\Set_{\perp}}
\newcommand{\UNFOLD}{\mathtt{UNFOLD}}
\newcommand{\Net}[1]{#1\text{-}\mathsf{Net}}
\newcommand{\Adj}{\mathbb{A}\mathsf{dj}}
\newcommand{\Csp}{\mathbb{C}\mathsf{sp}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\p}{\mathrm{p}}
\renewcommand{\r}{\mathrm{r}}
\newcommand{\ff}{f}

% objects
\newcommand{\stock}{\mathrm{stock}}
\newcommand{\flow}{\mathrm{flow}}
\newcommand{\link}{\mathrm{link}}
\newcommand{\variable}{\mathrm{variable}}
\newcommand{\sumvariable}{\mathrm{sum variable}}
\newcommand{\sumlink}{\mathrm{sum link}}

\newcommand{\Stock}{\mathrm{S}}
\newcommand{\Flow}{\mathrm{F}}
\newcommand{\Variable}{\mathrm{V}}
\newcommand{\SumVariable}{\mathrm{SV}}
\newcommand{\Inflow}{\mathrm{I}}
\newcommand{\Outflow}{\mathrm{O}}
\newcommand{\LS}{\mathrm{LS}}
\newcommand{\LV}{\mathrm{LV}}
\newcommand{\LSV}{\mathrm{LSV}}

% subscripts
\newcommand{\ICU}{\mathrm{ICU}}
\newcommand{\NICU}{\mathrm{NICU}}

\makeatletter
\newcommand*{\relrelbarsep}{.386ex}
\newcommand*{\relrelbar}{%
  \mathrel{%
    \mathpalette\@relrelbar\relrelbarsep
  }%
}
\newcommand*{\@relrelbar}[2]{%
  \raise#2\hbox to 0pt{$\m@th#1\relbar$\hss}%
  \lower#2\hbox{$\m@th#1\relbar$}%
}
\providecommand*{\rightrightarrowsfill@}{%
  \arrowfill@\relrelbar\relrelbar\rightrightarrows
}
\providecommand*{\leftleftarrowsfill@}{%
  \arrowfill@\leftleftarrows\relrelbar\relrelbar
}
\providecommand*{\xrightrightarrows}[2][]{%
  \ext@arrow 0359\rightrightarrowsfill@{#1}{#2}%
}
\providecommand*{\xleftleftarrows}[2][]{%
  \ext@arrow 3095\leftleftarrowsfill@{#1}{#2}%
}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\usepackage{subfiles}
%\usepackage{stackengine}
\usepackage{mathtools}
\usepackage[utf8]{inputenc}
\usepackage{csquotes}
\usepackage[a4paper,top=3cm,bottom=3cm,inner=3cm,outer=3cm]{geometry}

\usepackage{comment}

\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage[all,2cell]{xy}\UseAllTwocells\SilentMatrices
\definecolor{darkgreen}{rgb}{0,0.45,0}
%\usepackage[colorlinks,citecolor=darkgreen,urlcolor=gray,final,hyperindex,linktoc=page,pagebackref]{hyperref}

\usepackage[capitalize]{cleveref}
\crefname{equation}{}{}
\crefname{item}{}{}
\usepackage{enumerate}



\newtheorem*{thm*}{Theorem}
\theoremstyle{remark}
\newtheorem*{rmk*}{Remark}
\newtheorem*{lem*}{Lemma}
\theoremstyle{definition}
\newtheorem*{defn*}{Definition}
\newtheorem*{cor*}{Corollary}
\theoremstyle{definition}
\newtheorem*{examples*}{Examples}
\newtheorem{prop*}{Proposition}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\theoremstyle{plain}
\newtheorem{prop}[thm]{Proposition}
\theoremstyle{remark}
\newtheorem{rmk}[thm]{Remark}
\theoremstyle{plain}
\newtheorem{lem}[thm]{Lemma}
\theoremstyle{plain}
\newtheorem{cor}[thm]{Corollary}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\theoremstyle{definition}
\newtheorem{ex}[thm]{Example}










\newcommand{\maps}{\colon}




==> backup/references_sample.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} If the citatiion in the text is numbered, the reference list should be arranged in ascending order. If the citation in the text is author/year, the reference list should be \textit{sorted} alphabetically and if there are several works by the same author, the following order should be used:
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer Nature style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O'Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> juliaCodeAndExamples/paper_mfph_copy.tex <==
   

%\begin{document}
    
%    \maketitle
    
    
The codes below can be reached in the GitHub repository of: \url{https://github.com/Xiaoyan-Li/applicationStockFlowMFPH}   
    
    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{1}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{k}{using} \PY{n}{StockFlow}

\PY{k}{using} \PY{n}{Catlab}
\PY{k}{using} \PY{n}{Catlab}\PY{o}{.}\PY{n}{CategoricalAlgebra}
\PY{k}{using} \PY{n}{LabelledArrays}
\PY{k}{using} \PY{n}{OrdinaryDiffEq}
\PY{k}{using} \PY{n}{Plots}

\PY{k}{using} \PY{n}{Catlab}\PY{o}{.}\PY{n}{Graphics}
\PY{k}{using} \PY{n}{Catlab}\PY{o}{.}\PY{n}{Programs}
\PY{k}{using} \PY{n}{Catlab}\PY{o}{.}\PY{n}{WiringDiagrams}

\PY{k}{using} \PY{n}{Catlab}\PY{o}{.}\PY{n}{Graphics}\PY{o}{.}\PY{n}{Graphviz}\PY{o}{:} \PY{n}{Html}
\PY{k}{using} \PY{n}{Catlab}\PY{o}{.}\PY{n}{Graphics}\PY{o}{.}\PY{n}{Graphviz}
\end{Verbatim}
\end{tcolorbox}

    \hypertarget{seir-model}{%
\section{SEIR Model}\label{seir-model}}

\hypertarget{syntax-define-the-seir-stock-and-flow-diagram}{%
\subsection{Syntax: Define the SEIR Stock \& Flow
Diagram}\label{syntax-define-the-seir-stock-and-flow-diagram}}

    Builds the stock \& flow diagram of the SEIR model:
    
\begin{figure}
\centering
\includegraphics[width=0.8\columnwidth]{juliaCodeAndExamples/SEIR_stockflow.jpg}
\caption{stratifications.jpg}
\end{figure}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{2}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c}{\PYZsh{} define the functions of the auxiliary variables}
\PY{n}{f\PYZus{}birth}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{p}\PY{o}{.}\PY{n}{μ}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{N}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}
\PY{n}{f\PYZus{}incid}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=} \PY{n}{p}\PY{o}{.}\PY{n}{β}\PY{o}{*}\PY{n}{u}\PY{o}{.}\PY{n}{S}\PY{o}{*}\PY{n}{u}\PY{o}{.}\PY{n+nb}{I}\PY{o}{/}\PY{n}{uN}\PY{o}{.}\PY{n}{N}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}
\PY{n}{f\PYZus{}inf}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{E}\PY{o}{/}\PY{n}{p}\PY{o}{.}\PY{n}{tlatent}
\PY{n}{f\PYZus{}rec}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n+nb}{I}\PY{o}{/}\PY{n}{p}\PY{o}{.}\PY{n}{trecovery}
\PY{n}{f\PYZus{}deathS}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{S}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δ}
\PY{n}{f\PYZus{}deathE}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{E}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δ}
\PY{n}{f\PYZus{}deathI}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n+nb}{I}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δ}
\PY{n}{f\PYZus{}deathR}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{R}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δ}
\end{Verbatim}
\end{tcolorbox}

            \begin{tcolorbox}[breakable, size=fbox, boxrule=.5pt, pad at break*=1mm, opacityfill=0]
\prompt{Out}{outcolor}{2}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
f\_deathR (generic function with 1 method)
\end{Verbatim}
\end{tcolorbox}
        
    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{3}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seir}\PY{o}{=}\PY{n}{StockAndFlow}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{S}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{birth}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{incid}\PY{p}{,}\PY{o}{:}\PY{n}{deathS}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{p}{)}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{E}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{incid}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{inf}\PY{p}{,}\PY{o}{:}\PY{n}{deathE}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}inf}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathE}\PY{p}{)}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n+nb}{I}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{inf}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{rec}\PY{p}{,}\PY{o}{:}\PY{n}{deathI}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}rec}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{p}{)}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{R}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{rec}\PY{p}{,}\PY{o}{:}\PY{n}{deathR}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathR}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{birth}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birth}\PY{p}{,}\PY{o}{:}\PY{n}{incid}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,}\PY{o}{:}\PY{n}{inf}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}inf}\PY{p}{,}\PY{o}{:}\PY{n}{rec}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}rec}\PY{p}{,}\PY{o}{:}\PY{n}{deathS}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{p}{,}\PY{o}{:}\PY{n}{deathE}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathE}\PY{p}{,}\PY{o}{:}\PY{n}{deathI}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{p}{,}\PY{o}{:}\PY{n}{deathR}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathR}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}birth}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}birth}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}incid}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}inf}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}inf}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}rec}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}rec}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathS}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathE}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathE}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathI}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathR}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathR}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}birth}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{)}\PY{p}{)}
\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    We can also plot the SEIR stock \& flow diagram using the function
Graph() as below. This stock \& flow diagram is the same as the upper
figure. Although the software plotted diagrams may be not as
good as the upper figure, it will be improved in the future.

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{4}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{Graph}\PY{p}{(}\PY{n}{seir}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{4}{}
    
    \begin{center}    \adjustimage{max size={0.7\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_6_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{semantics-odes}{%
\subsection{Semantics: ODEs}\label{semantics-odes}}

    \hypertarget{define-the-constant-parameters-values-and-the-initial-values-of-the-stocks}{%
\subsubsection{Define the constant parameter values and the initial
values for the
stocks}\label{define-the-constant-parameters-values-and-the-initial-values-of-the-stocks}}

Time unit: Month

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{5}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c}{\PYZsh{} define parameter values and initial values of stocks}
\PY{c}{\PYZsh{} define constant parameters}
\PY{n}{p\PYZus{}measles} \PY{o}{=} \PY{n}{LVector}\PY{p}{(}
    \PY{n}{β}\PY{o}{=}\PY{l+m+mf}{49.598}\PY{p}{,} \PY{n}{μ}\PY{o}{=}\PY{l+m+mf}{0.03}\PY{o}{/}\PY{l+m+mi}{12}\PY{p}{,} \PY{n}{δ}\PY{o}{=}\PY{l+m+mf}{0.03}\PY{o}{/}\PY{l+m+mi}{12}\PY{p}{,} \PY{n}{tlatent}\PY{o}{=}\PY{l+m+mf}{8.0}\PY{o}{/}\PY{l+m+mi}{30}\PY{p}{,} \PY{n}{trecovery}\PY{o}{=}\PY{l+m+mf}{5.0}\PY{o}{/}\PY{l+m+mi}{30}
\PY{p}{)}
\PY{c}{\PYZsh{} define initial values for stocks}
\PY{n}{u0\PYZus{}measles} \PY{o}{=} \PY{n}{LVector}\PY{p}{(}
    \PY{n}{S}\PY{o}{=}\PY{l+m+mf}{90000.0}\PY{o}{\PYZhy{}}\PY{l+m+mf}{930.0}\PY{p}{,} \PY{n}{E}\PY{o}{=}\PY{l+m+mf}{0.0}\PY{p}{,} \PY{n+nb}{I}\PY{o}{=}\PY{l+m+mf}{930.0}\PY{p}{,} \PY{n}{R}\PY{o}{=}\PY{l+m+mf}{773545.0}
\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    \hypertarget{solve-the-odes-and-plot-the-results}{%
\subsubsection{Solve the ODEs and plot the
results}\label{solve-the-odes-and-plot-the-results}}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{6}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{prob\PYZus{}measles} \PY{o}{=} \PY{n}{ODEProblem}\PY{p}{(}\PY{n}{vectorfield}\PY{p}{(}\PY{n}{seir}\PY{p}{)}\PY{p}{,}\PY{n}{u0\PYZus{}measles}\PY{p}{,}\PY{p}{(}\PY{l+m+mf}{0.0}\PY{p}{,}\PY{l+m+mf}{120.0}\PY{p}{)}\PY{p}{,}\PY{n}{p\PYZus{}measles}\PY{p}{)}\PY{p}{;}
\PY{n}{sol\PYZus{}measles} \PY{o}{=} \PY{n}{solve}\PY{p}{(}\PY{n}{prob\PYZus{}measles}\PY{p}{,}\PY{n}{Tsit5}\PY{p}{(}\PY{p}{)}\PY{p}{,}\PY{n}{abstol}\PY{o}{=}\PY{l+m+mf}{1e\PYZhy{}8}\PY{p}{)}\PY{p}{;}
\PY{n}{plot}\PY{p}{(}\PY{n}{sol\PYZus{}measles}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{6}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_11_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{semantics-causal-loop-diagrams}{%
\subsection{Semantics: Causal Loop
Diagrams}\label{semantics-causal-loop-diagrams}}

\hypertarget{convert-the-seir-stock-and-flow-diagram-to-the-causal-loop-diagram}{%
\paragraph{Convert the SEIR stock \& flow diagram to the causal loop
diagram:}\label{convert-the-seir-stock-and-flow-diagram-to-the-causal-loop-diagram}}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{7}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seir\PYZus{}causalLoop}\PY{o}{=}\PY{n}{convertToCausalLoop}\PY{p}{(}\PY{n}{seir}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{8}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{Graph}\PY{p}{(}\PY{n}{seir\PYZus{}causalLoop}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{8}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_14_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{semantics-system-structure-diagrams}{%
\subsection{Semantics: System Structure
Diagrams}\label{semantics-system-structure-diagrams}}

\hypertarget{convert-the-seir-stock-and-flow-diagram-to-the-system-structure-diagram}{%
\paragraph{Convert the SEIR stock \& flow diagram to the System
Structure
diagram:}\label{convert-the-seir-stock-and-flow-diagram-to-the-system-structure-diagram}}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{9}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seir\PYZus{}structure}\PY{o}{=}\PY{n}{convertStockFlowToSystemStructure}\PY{p}{(}\PY{n}{seir}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{10}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{Graph}\PY{p}{(}\PY{n}{seir\PYZus{}structure}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{10}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_17_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{composition}{%
\section{Composition}\label{composition}}

    \hypertarget{open-population-sve-model}{%
\subsection{Open population SVE model}\label{open-population-sve-model}}

\begin{figure}
\centering
\includegraphics[width=0.4\columnwidth]{juliaCodeAndExamples/SEV_stockflow.jpg}
\caption{stratifications.jpg}
\end{figure}    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{11}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{f\PYZus{}vacc}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{S}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{α}
\PY{n}{f\PYZus{}deathV}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{V}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δ}
\PY{n}{f\PYZus{}incidv}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{p}\PY{o}{.}\PY{n}{β}\PY{o}{*}\PY{n}{u}\PY{o}{.}\PY{n}{V}\PY{o}{*}\PY{n}{u}\PY{o}{.}\PY{n+nb}{I}\PY{o}{*}\PY{p}{(}\PY{l+m+mf}{1.0}\PY{o}{\PYZhy{}}\PY{n}{p}\PY{o}{.}\PY{n+nb}{e}\PY{p}{)}\PY{o}{/}\PY{n}{uN}\PY{o}{.}\PY{n}{N}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}

\PY{n}{sve}\PY{o}{=}\PY{n}{StockAndFlow}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{S}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{F\PYZus{}NONE}\PY{p}{,}\PY{o}{:}\PY{n}{vacc}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}vacc}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{,} 
        \PY{o}{:}\PY{n}{V}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{vacc}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathV}\PY{p}{,}\PY{o}{:}\PY{n}{incidv}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathV}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}incidv}\PY{p}{)}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{,} 
        \PY{o}{:}\PY{n}{E}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{incidv}\PY{p}{,}\PY{o}{:}\PY{n}{F\PYZus{}NONE}\PY{p}{,}\PY{o}{:}\PY{n}{V\PYZus{}NONE}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n+nb}{I}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{F\PYZus{}NONE}\PY{p}{,}\PY{o}{:}\PY{n}{F\PYZus{}NONE}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}incidv}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{vacc}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}vacc}\PY{p}{,}\PY{o}{:}\PY{n}{deathV}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathV}\PY{p}{,} \PY{o}{:}\PY{n}{incidv}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}incidv}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}vacc}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}vacc}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathV}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathV}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}incidv}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}incidv}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}incidv}\PY{p}{)}
\PY{p}{)}

\PY{n}{Graph}\PY{p}{(}\PY{n}{sve}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{11}{}
    
    \begin{center}
    \adjustimage{max size={0.45\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_21_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{composition}{%
\subsection{Composition}\label{composition}}

    \hypertarget{define-the-composition-uwd-algebra}{%
\subsubsection{Define the composition
UWD-algebra}\label{define-the-composition-uwd-algebra}}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{12}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seirv\PYZus{}uwd} \PY{o}{=} \PY{n+nd}{@relation} \PY{p}{(}\PY{n}{S}\PY{p}{,}\PY{n}{E}\PY{p}{,}\PY{n+nb}{I}\PY{p}{)} \PY{k}{begin}
    \PY{n}{seir}\PY{p}{(}\PY{n}{S}\PY{p}{,}\PY{n}{E}\PY{p}{,}\PY{n+nb}{I}\PY{p}{)}
    \PY{n}{sve}\PY{p}{(}\PY{n}{S}\PY{p}{,}\PY{n}{E}\PY{p}{,}\PY{n+nb}{I}\PY{p}{)}
\PY{k}{end}\PY{p}{;}
\PY{n}{display\PYZus{}uwd}\PY{p}{(}\PY{n}{seirv\PYZus{}uwd}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{12}{}
    
    \begin{center}
    \adjustimage{max size={0.4\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_24_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{define-the-common-parts-feet-to-be-composed-of}{%
\subsubsection{Define the common parts (feet) to be composed
of}\label{define-the-common-parts-feet-to-be-composed-of}}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{13}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{footS}\PY{o}{=}\PY{n}{foot}\PY{p}{(}\PY{o}{:}\PY{n}{S}\PY{p}{,} \PY{o}{:}\PY{n}{N}\PY{p}{,} \PY{o}{:}\PY{n}{S}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{N}\PY{p}{)}
\PY{n}{Graph}\PY{p}{(}\PY{n}{footS}\PY{p}{;}\PY{n}{schema}\PY{o}{=}\PY{l+s}{\PYZdq{}}\PY{l+s}{C}\PY{l+s}{0}\PY{l+s}{\PYZdq{}}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{13}{}
    
    \begin{center}
    \adjustimage{max size={0.2\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_26_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{14}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{footE}\PY{o}{=}\PY{n}{foot}\PY{p}{(}\PY{o}{:}\PY{n}{E}\PY{p}{,} \PY{o}{:}\PY{n}{N}\PY{p}{,} \PY{o}{:}\PY{n}{E}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{N}\PY{p}{)}
\PY{n}{Graph}\PY{p}{(}\PY{n}{footE}\PY{p}{;}\PY{n}{schema}\PY{o}{=}\PY{l+s}{\PYZdq{}}\PY{l+s}{C}\PY{l+s}{0}\PY{l+s}{\PYZdq{}}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{14}{}
    
    \begin{center}
    \adjustimage{max size={0.2\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_27_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{15}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{footI}\PY{o}{=}\PY{n}{foot}\PY{p}{(}\PY{o}{:}\PY{n+nb}{I}\PY{p}{,} \PY{o}{:}\PY{n}{N}\PY{p}{,} \PY{o}{:}\PY{n+nb}{I}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{N}\PY{p}{)}
\PY{n}{Graph}\PY{p}{(}\PY{n}{footI}\PY{p}{;}\PY{n}{schema}\PY{o}{=}\PY{l+s}{\PYZdq{}}\PY{l+s}{C}\PY{l+s}{0}\PY{l+s}{\PYZdq{}}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{15}{}
    
    \begin{center}
    \adjustimage{max size={0.2\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_28_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{composition}{%
\subsubsection{Composition}\label{composition}}

\begin{figure}
\centering
\includegraphics[width=0.8\columnwidth]{juliaCodeAndExamples/SEIRV_stockflow.jpg}
\caption{stratifications.jpg}
\end{figure}    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{16}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c}{\PYZsh{} open SEIR and SVE stock \& flow diagram with the feet defined before}
\PY{n}{open\PYZus{}seir}\PY{o}{=}\PY{n}{Open}\PY{p}{(}\PY{n}{seir}\PY{p}{,} \PY{n}{footS}\PY{p}{,} \PY{n}{footE}\PY{p}{,} \PY{n}{footI}\PY{p}{)}
\PY{n}{open\PYZus{}sve}\PY{o}{=}\PY{n}{Open}\PY{p}{(}\PY{n}{sve}\PY{p}{,} \PY{n}{footS}\PY{p}{,} \PY{n}{footE}\PY{p}{,} \PY{n}{footI}\PY{p}{)}
\PY{c}{\PYZsh{} Compose those two models according the UWD\PYZhy{}algebra}
\PY{n}{open\PYZus{}seirv} \PY{o}{=} \PY{n}{oapply}\PY{p}{(}\PY{n}{seirv\PYZus{}uwd}\PY{p}{,} \PY{p}{[}\PY{n}{open\PYZus{}seir}\PY{p}{,} \PY{n}{open\PYZus{}sve}\PY{p}{]}\PY{p}{)}
\PY{c}{\PYZsh{} the composed closed stock \& flow diagram is the apex of the open stock \& flow diagram}
\PY{n}{seirv} \PY{o}{=} \PY{n}{apex}\PY{p}{(}\PY{n}{open\PYZus{}seirv}\PY{p}{)}
\PY{n}{Graph}\PY{p}{(}\PY{n}{seirv}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{16}{}
    
    \begin{center}
    \adjustimage{max size={0.7\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_31_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{solve-the-odes-of-the-seirv-model}{%
\subsubsection{Solve the ODEs of the SEIRV
model}\label{solve-the-odes-of-the-seirv-model}}

Time Unit: days

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{17}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{p\PYZus{}seirv} \PY{o}{=} \PY{n}{LVector}\PY{p}{(}
    \PY{n}{β}\PY{o}{=}\PY{l+m+mf}{49.598}\PY{o}{/}\PY{l+m+mi}{30}\PY{p}{,} \PY{n}{μ}\PY{o}{=}\PY{l+m+mf}{0.03}\PY{o}{/}\PY{l+m+mi}{365}\PY{p}{,} \PY{n}{δ}\PY{o}{=}\PY{l+m+mf}{0.03}\PY{o}{/}\PY{l+m+mi}{365}\PY{p}{,} \PY{n}{tlatent}\PY{o}{=}\PY{l+m+mf}{8.0}\PY{p}{,} \PY{n}{trecovery}\PY{o}{=}\PY{l+m+mf}{5.0}\PY{p}{,} \PY{n}{α}\PY{o}{=}\PY{l+m+mf}{0.01}\PY{p}{,} \PY{n+nb}{e}\PY{o}{=}\PY{l+m+mf}{0.9}
\PY{p}{)}
\PY{c}{\PYZsh{} define initial values for stocks}
\PY{n}{u0\PYZus{}seirv} \PY{o}{=} \PY{n}{LVector}\PY{p}{(}
    \PY{n}{S}\PY{o}{=}\PY{l+m+mf}{10000.0}\PY{o}{\PYZhy{}}\PY{l+m+mf}{1.0}\PY{p}{,} \PY{n}{E}\PY{o}{=}\PY{l+m+mf}{0.0}\PY{p}{,} \PY{n+nb}{I}\PY{o}{=}\PY{l+m+mf}{1.0}\PY{p}{,} \PY{n}{R}\PY{o}{=}\PY{l+m+mf}{0.0}\PY{p}{,} \PY{n}{V}\PY{o}{=}\PY{l+m+mf}{0.0}
\PY{p}{)}\PY{p}{;}

\PY{n}{prob\PYZus{}seirv} \PY{o}{=} \PY{n}{ODEProblem}\PY{p}{(}\PY{n}{vectorfield}\PY{p}{(}\PY{n}{seirv}\PY{p}{)}\PY{p}{,}\PY{n}{u0\PYZus{}seirv}\PY{p}{,}\PY{p}{(}\PY{l+m+mf}{0.0}\PY{p}{,}\PY{l+m+mf}{100.0}\PY{p}{)}\PY{p}{,}\PY{n}{p\PYZus{}seirv}\PY{p}{)}\PY{p}{;}
\PY{n}{sol\PYZus{}seirv} \PY{o}{=} \PY{n}{solve}\PY{p}{(}\PY{n}{prob\PYZus{}seirv}\PY{p}{,}\PY{n}{Tsit5}\PY{p}{(}\PY{p}{)}\PY{p}{,}\PY{n}{abstol}\PY{o}{=}\PY{l+m+mf}{1e\PYZhy{}8}\PY{p}{)}\PY{p}{;}
\PY{n}{plot}\PY{p}{(}\PY{n}{sol\PYZus{}seirv}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{17}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_33_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{stratification}{%
\section{Stratification}\label{stratification}}

    define functions of the typed stock \& flow diagrams:

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{18}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c}{\PYZsh{} Functions for graphing typed stock \& flow diagrams}
\PY{n}{colors\PYZus{}vflow} \PY{o}{=} \PY{p}{[}\PY{l+s}{\PYZdq{}}\PY{l+s}{a}\PY{l+s}{n}\PY{l+s}{t}\PY{l+s}{i}\PY{l+s}{q}\PY{l+s}{u}\PY{l+s}{e}\PY{l+s}{w}\PY{l+s}{h}\PY{l+s}{i}\PY{l+s}{t}\PY{l+s}{e}\PY{l+s}{4}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{a}\PY{l+s}{n}\PY{l+s}{t}\PY{l+s}{i}\PY{l+s}{q}\PY{l+s}{u}\PY{l+s}{e}\PY{l+s}{w}\PY{l+s}{h}\PY{l+s}{i}\PY{l+s}{t}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{g}\PY{l+s}{o}\PY{l+s}{l}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{s}\PY{l+s}{a}\PY{l+s}{d}\PY{l+s}{d}\PY{l+s}{l}\PY{l+s}{e}\PY{l+s}{b}\PY{l+s}{r}\PY{l+s}{o}\PY{l+s}{w}\PY{l+s}{n}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{s}\PY{l+s}{l}\PY{l+s}{a}\PY{l+s}{t}\PY{l+s}{e}\PY{l+s}{b}\PY{l+s}{l}\PY{l+s}{u}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{b}\PY{l+s}{l}\PY{l+s}{u}\PY{l+s}{e}\PY{l+s}{v}\PY{l+s}{i}\PY{l+s}{o}\PY{l+s}{l}\PY{l+s}{e}\PY{l+s}{t}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{o}\PY{l+s}{l}\PY{l+s}{i}\PY{l+s}{v}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{]}
\PY{n}{colors\PYZus{}s} \PY{o}{=} \PY{p}{[}\PY{l+s}{\PYZdq{}}\PY{l+s}{d}\PY{l+s}{e}\PY{l+s}{e}\PY{l+s}{p}\PY{l+s}{p}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{k}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{d}\PY{l+s}{a}\PY{l+s}{r}\PY{l+s}{k}\PY{l+s}{o}\PY{l+s}{r}\PY{l+s}{c}\PY{l+s}{h}\PY{l+s}{i}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{d}\PY{l+s}{a}\PY{l+s}{r}\PY{l+s}{k}\PY{l+s}{r}\PY{l+s}{e}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{o}\PY{l+s}{r}\PY{l+s}{a}\PY{l+s}{l}\PY{l+s}{\PYZdq{}}\PY{p}{]} \PY{c}{\PYZsh{} red series}
\PY{n}{colors\PYZus{}sv} \PY{o}{=} \PY{p}{[}\PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{o}\PY{l+s}{r}\PY{l+s}{n}\PY{l+s}{f}\PY{l+s}{l}\PY{l+s}{o}\PY{l+s}{w}\PY{l+s}{e}\PY{l+s}{r}\PY{l+s}{b}\PY{l+s}{l}\PY{l+s}{u}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{y}\PY{l+s}{a}\PY{l+s}{n}\PY{l+s}{4}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{y}\PY{l+s}{a}\PY{l+s}{n}\PY{l+s}{\PYZdq{}}\PY{p}{,}\PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{h}\PY{l+s}{a}\PY{l+s}{r}\PY{l+s}{t}\PY{l+s}{r}\PY{l+s}{e}\PY{l+s}{u}\PY{l+s}{s}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{]} \PY{c}{\PYZsh{} green and blue series}

\PY{n}{flatten}\PY{p}{(}\PY{n}{fname}\PY{o}{::}\PY{k+kt}{Symbol}\PY{p}{)} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}fname}\PY{l+s}{\PYZdq{}}

\PY{k}{function} \PY{n}{flatten}\PY{p}{(}\PY{n}{fname}\PY{o}{::}\PY{k+kt}{Tuple}\PY{p}{)}
    \PY{n}{names} \PY{o}{=} \PY{n}{split}\PY{p}{(}\PY{n}{replace}\PY{p}{(}\PY{n}{string}\PY{p}{(}\PY{n}{fname}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{(}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{)}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{,}\PY{l+s}{\PYZdq{}}\PY{p}{)}
    \PY{k}{for} \PY{n}{i} \PY{k+kp}{in} \PY{l+m+mi}{1}\PY{o}{:}\PY{n}{length}\PY{p}{(}\PY{n}{names}\PY{p}{)}
        \PY{n}{name} \PY{o}{=} \PY{n}{strip}\PY{p}{(}\PY{n}{names}\PY{p}{[}\PY{n}{i}\PY{p}{]}\PY{p}{)}
        \PY{k}{if} \PY{n}{name}\PY{p}{[}\PY{l+m+mi}{1}\PY{o}{:}\PY{l+m+mi}{2}\PY{p}{]} \PY{o}{==} \PY{l+s}{\PYZdq{}}\PY{l+s}{i}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}
            \PY{k}{continue}
        \PY{k}{end}
        \PY{k}{return} \PY{n}{name}
    \PY{k}{end}
    \PY{k}{return} \PY{l+s}{\PYZdq{}}\PY{l+s}{i}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}
\PY{k}{end}

\PY{n}{def\PYZus{}stock}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{o}{::}\PY{n}{ACSetTransformation}\PY{p}{,} \PY{n}{colors}\PY{p}{)} \PY{o}{=} 
  \PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{s}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{s}\PY{l+s+si}{\PYZdl{}s}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{sname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{s}\PY{p}{)} \PY{k+kp}{isa} \PY{k+kt}{Tuple} \PY{n}{where} \PY{n}{T} \PY{o}{?} \PY{n}{Html}\PY{p}{(}\PY{n}{replace}\PY{p}{(}\PY{n}{string}\PY{p}{(}\PY{n}{sname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{s}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{,}\PY{l+s}{\PYZdq{}} \PY{o}{=\PYZgt{}} \PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZlt{}}\PY{l+s}{B}\PY{l+s}{R}\PY{l+s}{/}\PY{l+s}{\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{(}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{)}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}}\PY{p}{(}\PY{n}{sname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{s}\PY{p}{)}\PY{p}{)}\PY{l+s}{\PYZdq{}}\PY{p}{,}
                                     \PY{o}{:}\PY{n}{shape}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{s}\PY{l+s}{q}\PY{l+s}{u}\PY{l+s}{a}\PY{l+s}{r}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{,} 
                                     \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{b}\PY{l+s}{l}\PY{l+s}{a}\PY{l+s}{c}\PY{l+s}{k}\PY{l+s}{\PYZdq{}}\PY{p}{,} 
                                     \PY{o}{:}\PY{n}{style}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{f}\PY{l+s}{i}\PY{l+s}{l}\PY{l+s}{l}\PY{l+s}{e}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}\PY{p}{,} 
                                     \PY{o}{:}\PY{n}{fillcolor}\PY{o}{=\PYZgt{}}\PY{n}{colors}\PY{p}{[}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{[}\PY{o}{:}\PY{n}{S}\PY{p}{]}\PY{p}{(}\PY{n}{s}\PY{p}{)}\PY{p}{]}\PY{p}{)}\PY{p}{)}

\PY{n}{def\PYZus{}auxiliaryV}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{o}{::}\PY{n}{ACSetTransformation}\PY{p}{,} \PY{n}{colors}\PY{p}{)}\PY{o}{=}
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{v}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}v}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{vname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{)} \PY{k+kp}{isa} \PY{k+kt}{Tuple} \PY{n}{where} \PY{n}{T} \PY{o}{?} \PY{n}{Html}\PY{p}{(}\PY{n}{replace}\PY{p}{(}\PY{n}{string}\PY{p}{(}\PY{n}{vname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{,}\PY{l+s}{\PYZdq{}} \PY{o}{=\PYZgt{}} \PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZlt{}}\PY{l+s}{B}\PY{l+s}{R}\PY{l+s}{/}\PY{l+s}{\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{(}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{)}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}}\PY{p}{(}\PY{n}{vname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{)}\PY{p}{)}\PY{l+s}{\PYZdq{}}\PY{p}{,}
                                          \PY{o}{:}\PY{n}{shape}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{p}\PY{l+s}{l}\PY{l+s}{a}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{t}\PY{l+s}{e}\PY{l+s}{x}\PY{l+s}{t}\PY{l+s}{\PYZdq{}}\PY{p}{,} 
                                          \PY{o}{:}\PY{n}{fontcolor}\PY{o}{=\PYZgt{}}\PY{n}{colors}\PY{p}{[}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{[}\PY{o}{:}\PY{n}{F}\PY{p}{]}\PY{p}{(}\PY{n}{incident}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{,}\PY{o}{:}\PY{n}{fv}\PY{p}{)}\PY{o}{.}\PY{o}{.}\PY{o}{.}\PY{p}{)}\PY{p}{]}\PY{p}{)}\PY{p}{)}


\PY{n}{def\PYZus{}auxiliaryV}\PY{p}{(}\PY{n}{colors} \PY{o}{=} \PY{n}{colors\PYZus{}vflow}\PY{p}{)}\PY{o}{=}
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{v}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}v}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{vname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{)} \PY{k+kp}{isa} \PY{k+kt}{Tuple} \PY{n}{where} \PY{n}{T} \PY{o}{?} \PY{n}{Html}\PY{p}{(}\PY{n}{replace}\PY{p}{(}\PY{n}{string}\PY{p}{(}\PY{n}{vname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{,}\PY{l+s}{\PYZdq{}} \PY{o}{=\PYZgt{}} \PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZlt{}}\PY{l+s}{B}\PY{l+s}{R}\PY{l+s}{/}\PY{l+s}{\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{(}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{)}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}}\PY{p}{(}\PY{n}{vname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{)}\PY{p}{)}\PY{l+s}{\PYZdq{}}\PY{p}{,}
                                          \PY{o}{:}\PY{n}{shape}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{p}\PY{l+s}{l}\PY{l+s}{a}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{t}\PY{l+s}{e}\PY{l+s}{x}\PY{l+s}{t}\PY{l+s}{\PYZdq{}}\PY{p}{,} 
                                          \PY{o}{:}\PY{n}{fontcolor}\PY{o}{=\PYZgt{}}\PY{n}{colors}\PY{p}{[}\PY{n}{incident}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{v}\PY{p}{,}\PY{o}{:}\PY{n}{fv}\PY{p}{)}\PY{o}{.}\PY{o}{.}\PY{o}{.}\PY{p}{]}\PY{p}{)}\PY{p}{)}



\PY{n}{def\PYZus{}sumV}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{o}{::}\PY{n}{ACSetTransformation}\PY{p}{,} \PY{n}{colors}\PY{p}{)} \PY{o}{=} 
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{sv}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{p}{(}\PY{l+s}{\PYZdq{}}\PY{l+s}{s}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}sv}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{svname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{sv}\PY{p}{)} \PY{k+kp}{isa} \PY{k+kt}{Tuple} \PY{n}{where} \PY{n}{T} \PY{o}{?} \PY{n}{Html}\PY{p}{(}\PY{n}{replace}\PY{p}{(}\PY{n}{string}\PY{p}{(}\PY{n}{svname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{sv}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{,}\PY{l+s}{\PYZdq{}} \PY{o}{=\PYZgt{}} \PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZlt{}}\PY{l+s}{B}\PY{l+s}{R}\PY{l+s}{/}\PY{l+s}{\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{(}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{)}\PY{l+s}{\PYZdq{}}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)} \PY{o}{:} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}}\PY{p}{(}\PY{n}{svname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{sv}\PY{p}{)}\PY{p}{)}\PY{l+s}{\PYZdq{}}\PY{p}{,}
                                       \PY{o}{:}\PY{n}{shape}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{c}\PY{l+s}{i}\PY{l+s}{r}\PY{l+s}{c}\PY{l+s}{l}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}\PY{p}{,} 
                                       \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{b}\PY{l+s}{l}\PY{l+s}{a}\PY{l+s}{c}\PY{l+s}{k}\PY{l+s}{\PYZdq{}}\PY{p}{,}
                                       \PY{o}{:}\PY{n}{fillcolor}\PY{o}{=\PYZgt{}}\PY{n}{colors}\PY{p}{[}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{[}\PY{o}{:}\PY{n}{SV}\PY{p}{]}\PY{p}{(}\PY{n}{sv}\PY{p}{)}\PY{p}{]}\PY{p}{,} 
                                       \PY{o}{:}\PY{n}{style}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{f}\PY{l+s}{i}\PY{l+s}{l}\PY{l+s}{l}\PY{l+s}{e}\PY{l+s}{d}\PY{l+s}{\PYZdq{}}\PY{p}{)}\PY{p}{)}  


\PY{n}{def\PYZus{}flow\PYZus{}V}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{o}{::}\PY{n}{ACSetTransformation}\PY{p}{,} \PY{n}{colors}\PY{p}{)}\PY{o}{=}
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{us}\PY{p}{,} \PY{n}{ds}\PY{p}{,} \PY{n}{v}\PY{p}{,} \PY{n}{f}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{k}{begin}
    \PY{n}{labelfontsize} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s}{6}\PY{l+s}{\PYZdq{}}
    \PY{n}{colorType} \PY{o}{=} \PY{n}{colors}\PY{p}{[}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{[}\PY{o}{:}\PY{n}{F}\PY{p}{]}\PY{p}{(}\PY{n}{f}\PY{p}{)}\PY{p}{]}
    \PY{n}{color} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{v}\PY{l+s}{i}\PY{l+s}{s}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}
    \PY{n}{arrowhead} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s}{n}\PY{l+s}{o}\PY{l+s}{n}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}
    \PY{n}{splines} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s}{o}\PY{l+s}{r}\PY{l+s}{t}\PY{l+s}{h}\PY{l+s}{o}\PY{l+s}{\PYZdq{}}
    \PY{k}{return} \PY{p}{(}\PY{p}{[}\PY{n}{us}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}v}\PY{l+s}{\PYZdq{}}\PY{p}{]}\PY{p}{,}\PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{o}{:}\PY{n}{labelfontsize}\PY{o}{=\PYZgt{}}\PY{n}{labelfontsize}\PY{p}{,} \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{n}{color}\PY{p}{,} \PY{o}{:}\PY{n}{arrowhead}\PY{o}{=\PYZgt{}}\PY{n}{arrowhead}\PY{p}{,} \PY{o}{:}\PY{n}{splines}\PY{o}{=\PYZgt{}}\PY{n}{splines}\PY{p}{)}\PY{p}{)}\PY{p}{,}
           \PY{p}{(}\PY{p}{[}\PY{l+s}{\PYZdq{}}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}v}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{ds}\PY{p}{]}\PY{p}{,}\PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{Html}\PY{p}{(}\PY{n}{flatten}\PY{p}{(}\PY{n}{fname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{f}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{labelfontsize}\PY{o}{=\PYZgt{}}\PY{n}{labelfontsize}\PY{p}{,} \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{n}{color}\PY{p}{,} \PY{o}{:}\PY{n}{splines}\PY{o}{=\PYZgt{}}\PY{n}{splines}\PY{p}{)}\PY{p}{)}            
\PY{k}{end}
        
\PY{n}{def\PYZus{}flow\PYZus{}noneV}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{o}{::}\PY{n}{ACSetTransformation}\PY{p}{,} \PY{n}{colors}\PY{p}{)}\PY{o}{=}
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{us}\PY{p}{,} \PY{n}{ds}\PY{p}{,} \PY{n}{f}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{k}{begin}
     \PY{n}{colorType} \PY{o}{=} \PY{n}{colors}\PY{p}{[}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{[}\PY{o}{:}\PY{n}{F}\PY{p}{]}\PY{p}{(}\PY{n}{f}\PY{p}{)}\PY{p}{]}
     \PY{n}{color} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{v}\PY{l+s}{i}\PY{l+s}{s}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}   
     \PY{p}{(}\PY{p}{[}\PY{n}{us}\PY{p}{,} \PY{n}{ds}\PY{p}{]}\PY{p}{,}\PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{Html}\PY{p}{(}\PY{n}{flatten}\PY{p}{(}\PY{n}{fname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{f}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{labelfontsize}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{6}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{n}{color}\PY{p}{)}\PY{p}{)}
\PY{k}{end}

\PY{n}{def\PYZus{}flow\PYZus{}V}\PY{p}{(}\PY{n}{colors} \PY{o}{=} \PY{n}{colors\PYZus{}vflow}\PY{p}{)}\PY{o}{=}
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{us}\PY{p}{,} \PY{n}{ds}\PY{p}{,} \PY{n}{v}\PY{p}{,} \PY{n}{f}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{k}{begin}
    \PY{n}{labelfontsize} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s}{6}\PY{l+s}{\PYZdq{}}
    \PY{n}{colorType} \PY{o}{=} \PY{n}{colors}\PY{p}{[}\PY{n}{f}\PY{p}{]}
    \PY{n}{color} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{v}\PY{l+s}{i}\PY{l+s}{s}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}
    \PY{n}{arrowhead} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s}{n}\PY{l+s}{o}\PY{l+s}{n}\PY{l+s}{e}\PY{l+s}{\PYZdq{}}
    \PY{n}{splines} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s}{o}\PY{l+s}{r}\PY{l+s}{t}\PY{l+s}{h}\PY{l+s}{o}\PY{l+s}{\PYZdq{}}
    \PY{k}{return} \PY{p}{(}\PY{p}{[}\PY{n}{us}\PY{p}{,} \PY{l+s}{\PYZdq{}}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}v}\PY{l+s}{\PYZdq{}}\PY{p}{]}\PY{p}{,}\PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{o}{:}\PY{n}{labelfontsize}\PY{o}{=\PYZgt{}}\PY{n}{labelfontsize}\PY{p}{,} \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{n}{color}\PY{p}{,} \PY{o}{:}\PY{n}{arrowhead}\PY{o}{=\PYZgt{}}\PY{n}{arrowhead}\PY{p}{,} \PY{o}{:}\PY{n}{splines}\PY{o}{=\PYZgt{}}\PY{n}{splines}\PY{p}{)}\PY{p}{)}\PY{p}{,}
           \PY{p}{(}\PY{p}{[}\PY{l+s}{\PYZdq{}}\PY{l+s}{v}\PY{l+s+si}{\PYZdl{}v}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{ds}\PY{p}{]}\PY{p}{,}\PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{Html}\PY{p}{(}\PY{n}{flatten}\PY{p}{(}\PY{n}{fname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{f}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{labelfontsize}\PY{o}{=\PYZgt{}}\PY{n}{labelfontsize}\PY{p}{,} \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{n}{color}\PY{p}{,} \PY{o}{:}\PY{n}{splines}\PY{o}{=\PYZgt{}}\PY{n}{splines}\PY{p}{)}\PY{p}{)}            
    
\PY{k}{end}
        
\PY{n}{def\PYZus{}flow\PYZus{}noneV}\PY{p}{(}\PY{n}{colors} \PY{o}{=} \PY{n}{colors\PYZus{}vflow}\PY{p}{)}\PY{o}{=}
  \PY{p}{(}\PY{n}{p}\PY{p}{,} \PY{n}{us}\PY{p}{,} \PY{n}{ds}\PY{p}{,} \PY{n}{f}\PY{p}{)} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{k}{begin}
     \PY{n}{colorType} \PY{o}{=} \PY{n}{colors}\PY{p}{[}\PY{n}{f}\PY{p}{]}
     \PY{n}{color} \PY{o}{=} \PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s}{:}\PY{l+s}{i}\PY{l+s}{n}\PY{l+s}{v}\PY{l+s}{i}\PY{l+s}{s}\PY{l+s}{:}\PY{l+s}{\PYZdq{}}\PY{o}{*}\PY{l+s}{\PYZdq{}}\PY{l+s+si}{\PYZdl{}colorType}\PY{l+s}{\PYZdq{}}   
     \PY{p}{(}\PY{p}{[}\PY{n}{us}\PY{p}{,} \PY{n}{ds}\PY{p}{]}\PY{p}{,}\PY{n}{Attributes}\PY{p}{(}\PY{o}{:}\PY{n}{label}\PY{o}{=\PYZgt{}}\PY{n}{Html}\PY{p}{(}\PY{n}{flatten}\PY{p}{(}\PY{n}{fname}\PY{p}{(}\PY{n}{p}\PY{p}{,}\PY{n}{f}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{labelfontsize}\PY{o}{=\PYZgt{}}\PY{l+s}{\PYZdq{}}\PY{l+s}{6}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{o}{:}\PY{n}{color}\PY{o}{=\PYZgt{}}\PY{n}{color}\PY{p}{)}\PY{p}{)}
\PY{k}{end}

\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{o}{::}\PY{n}{ACSetTransformation}\PY{p}{,} \PY{n}{colors\PYZus{}vflow} \PY{o}{=} \PY{n}{colors\PYZus{}vflow}\PY{p}{,} \PY{n}{colors\PYZus{}s} \PY{o}{=} \PY{n}{colors\PYZus{}s}\PY{p}{,} \PY{n}{colors\PYZus{}sv} \PY{o}{=} \PY{n}{colors\PYZus{}sv}\PY{p}{;} \PY{n}{schema}\PY{o}{::}\PY{n}{String}\PY{o}{=}\PY{l+s}{\PYZdq{}}\PY{l+s}{C}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{k}{type}\PY{o}{::}\PY{n}{String}\PY{o}{=}\PY{l+s}{\PYZdq{}}\PY{l+s}{S}\PY{l+s}{F}\PY{l+s}{V}\PY{l+s}{L}\PY{l+s}{\PYZdq{}}\PY{p}{,} \PY{n}{rd}\PY{o}{::}\PY{n}{String}\PY{o}{=}\PY{l+s}{\PYZdq{}}\PY{l+s}{L}\PY{l+s}{R}\PY{l+s}{\PYZdq{}}\PY{p}{)} \PY{o}{=} \PY{n}{Graph}\PY{p}{(}\PY{n}{dom}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{)}\PY{p}{,}
    \PY{n}{make\PYZus{}stock} \PY{o}{=} \PY{n}{def\PYZus{}stock}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{,} \PY{n}{colors\PYZus{}s}\PY{p}{)}\PY{p}{,} \PY{n}{make\PYZus{}auxiliaryV}\PY{o}{=}\PY{n}{def\PYZus{}auxiliaryV}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{,} \PY{n}{colors\PYZus{}vflow}\PY{p}{)}\PY{p}{,} \PY{n}{make\PYZus{}sumV}\PY{o}{=}\PY{n}{def\PYZus{}sumV}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{,} \PY{n}{colors\PYZus{}sv}\PY{p}{)}\PY{p}{,} 
    \PY{n}{make\PYZus{}flow\PYZus{}V}\PY{o}{=}\PY{n}{def\PYZus{}flow\PYZus{}V}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{,} \PY{n}{colors\PYZus{}vflow}\PY{p}{)}\PY{p}{,} \PY{n}{make\PYZus{}flow\PYZus{}noneV}\PY{o}{=}\PY{n}{def\PYZus{}flow\PYZus{}noneV}\PY{p}{(}\PY{n}{typed\PYZus{}StockFlow}\PY{p}{,} \PY{n}{colors\PYZus{}vflow}\PY{p}{)}\PY{p}{,}\PY{n}{schema}\PY{o}{=}\PY{n}{schema}\PY{p}{,} \PY{k}{type}\PY{o}{=}\PY{k}{type}\PY{p}{,} \PY{n}{rd}\PY{o}{=}\PY{n}{rd}
\PY{p}{)}
            
\PY{c}{\PYZsh{} Plot the typed stock \& flow diagram}
\PY{n}{stratify}\PY{p}{(}\PY{n}{typed\PYZus{}models}\PY{o}{.}\PY{o}{.}\PY{o}{.}\PY{p}{)} \PY{o}{=} \PY{n}{ob}\PY{p}{(}\PY{n}{pullback}\PY{p}{(}\PY{n}{collect}\PY{p}{(}\PY{n}{typed\PYZus{}models}\PY{p}{)}\PY{p}{)}\PY{p}{)}

\PY{n}{typed\PYZus{}stratify}\PY{p}{(}\PY{n}{typed\PYZus{}models}\PY{o}{.}\PY{o}{.}\PY{o}{.}\PY{p}{)} \PY{o}{=}
  \PY{n}{compose}\PY{p}{(}\PY{n}{legs}\PY{p}{(}\PY{n}{pullback}\PY{p}{(}\PY{n}{collect}\PY{p}{(}\PY{n}{typed\PYZus{}models}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{p}{,} \PY{n}{typed\PYZus{}models}\PY{p}{[}\PY{l+m+mi}{1}\PY{p}{]}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    \hypertarget{stratification}{%
\subsection{Stratification}\label{stratification}}

    The stratification is based on the system structure diagrams. The stratified stock \& flow
diagrams are then generated by assigning functions to each auxiliary
variables of the stratified system structure diagrams.

The stratified system structure diagrams are generated from the pullback
of the aggregate population infectious disease system structure diagram
(labelled as \(S_{Aggregate}\)) and the strata system structure diagram
(labelled as \(S_{Strata}\)) based on the same co-domain of the typed
system structure diagram (labelled as \(S_{Typed}\)). The pullback
\(S_{Stratified}\) of \(S_{Aggregate}\) and \(S_{Strata}\) is the
stratified diagrams to be built, and written mathematically as
\(S_{Stratified}=S_{Aggregate} \times_{S_{Typed}} S_{Strata}\). The
pullback square is as follows:

\begin{figure}
\centering
\includegraphics[width=0.35\columnwidth]{juliaCodeAndExamples/pullback_square.jpg}
\caption{stratifications.jpg}
\end{figure}    

    The morphism \(t_{aggregte}\) is the map
(\(S_{Aggregate} \rightarrow S_{Typed}\)) from the system structure
diagram \(S_{Aggregate}\) to the typed system 
\(S_{Typed}\). Basically, we can think of \(t_{aggregate}\) as the
system structure diagram \(S_{Aggregate}\) with extra information of
having each part assigned a type. The type is based on the typed
system \(S_{Typed}\). The same as the morphism of
\(t_{strata}\) -- the map (\(S_{Strata} \rightarrow S_{Typed}\)) from
the system structure diagram \(S_{Strata}\) to \(S_{Typed}\).

In the application, we can define multiple models of the
\(S_{Aggregate}\) system structure diagram to represent different
infectious disease models (or more generally, compartmental models),
e.g., the SEIR (Susceptible-Exposed-Infectious-Recovered) model, SIR
(Susceptible-Infectious-Recovered) model, SIS
(Susceptible-Infectious-Susceptible) model, etc. Similarly, the strata
system structure diagrams \(S_{Strata}\) are consist of multiple different
strata models, e.g., the age strata, the sex strata, the region strata,
etc. Then, a stratified model can be build by calculating the pullback
of a disease model of the \(S_{Aggregate}\) and a strata model of the
\(S_{Strata}\). For example, we can generate a SEIR age stratified
system structure diagram by calculating the pullback of the disease SEIR
model, and the age strata model.

In this project, we have built two strata models (age strata model, and
sex strata model), and two disease models (SEIR model, and SIS model) as
examples. Finally, four stratified models are generated by calculating
the pullback of the four different combination of the two strata models
and two disease models. Those four built stratified models by pullback
are age stratified SEIR model, age stratified SIS model, sex stratified
SEIR model and sex stratified SIS model. The examples are listed as
follows:

    \begin{figure}
\centering
\includegraphics[width=1.05\columnwidth]{juliaCodeAndExamples/stratifications.jpg}
\caption{stratifications.jpg}
\end{figure}

    \hypertarget{define-the-typed-system-structure-diagram}{%
\subsubsection{Define the typed system structure
diagram}\label{define-the-typed-system-structure-diagram}}

    Firstly, we need to define the typed system structure diagram of
\(S_{Typed}\). In this typed system structure diagram, each component
represents a type.

    \begin{figure}
\centering
\includegraphics[width=0.4\columnwidth]{juliaCodeAndExamples/s_type.png}
\caption{stratifications.jpg}
\end{figure}


The typed system structure diagram used in this project is shown in the
upper figure. From the figure we can see there is only a unique type
of stock which represent population. There are 5 flows in this diagram.
Those 5 flows represent 5 different flow types in the infectious disease
models. And they are plotted using different colors to have a clearer
visulization: 

- the birth flow 

- the death flow 

- the flow of new infectious

- the aging flow which represents the flow of aging from one age
group to the elder group 

- the first order delay flow 

Based on the schema of the system structure diagrams, there should be 5 types of
auxiliary variables corresponds to those 5 flows, and having one to one
correspondence. We did not plot out those 5 auxiliary variables for simplicity.

There are 3 different types of sum auxiliary variables: 

- \(N\):
represents the total population of the whole model 

- \(NS\): represents
the total population of a specific subgroup 

- \(NI\): represents the
total infectious of a specific subgroup

Each link in the typed system structure diagram also represents a type
of link. However, since we can easily check a link's type by its
source's and target's type, we did not label the links type by colors
for simplicity.

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{19}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{S\PYZus{}type}\PY{o}{=}\PY{n}{StockAndFlowStructure}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{Pop}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{births}\PY{p}{,} \PY{o}{:}\PY{n}{newInfectious}\PY{p}{,} \PY{o}{:}\PY{n}{firstOrderDelay}\PY{p}{,} \PY{o}{:}\PY{n}{aging}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deaths}\PY{p}{,} \PY{o}{:}\PY{n}{newInfectious}\PY{p}{,} \PY{o}{:}\PY{n}{firstOrderDelay}\PY{p}{,} \PY{o}{:}\PY{n}{aging}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}aging}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NS}\PY{p}{,}\PY{o}{:}\PY{n}{NI}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{deaths}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{o}{:}\PY{n}{births}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{o}{:}\PY{n}{newInfectious}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{o}{:}\PY{n}{firstOrderDelay}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{o}{:}\PY{n}{aging}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}aging}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{o}{:}\PY{n}{NI}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{o}{:}\PY{n}{NS}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{)}
\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{id}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{)}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{19}{}
    
    \begin{center}
    \adjustimage{max size={0.4\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_46_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{20}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c}{\PYZsh{} eliminate the attribute of name to enable pass the natural check}
\PY{n}{S\PYZus{}type} \PY{o}{=} \PY{n}{map}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{n}{Name}\PY{o}{=}\PY{n}{name}\PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}}\PY{n+nb}{nothing}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    Since the typed disease model (e.g., SEIR model) and typed strata model
(e.g., age strata, sex strata) are homomorphisms (with
ACSetTransformation data structure) from disease (e.g., SEIR) system
structure diagrams or the strata system structure diagrams to the typed
system structure diagram. To define the ACSetTransformation easily, we
extract the parts of each components of the typed system structure
diagram as follows:

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{21}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{s}\PY{p}{,} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{S}\PY{p}{)}
\PY{n}{sv\PYZus{}N}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{SV}\PY{p}{)}
\PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}N} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{LS}\PY{p}{)}
\PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}aging} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{F}\PY{p}{)}
\PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n+nb}{I}\PY{p}{)}
\PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}aging} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{O}\PY{p}{)}
\PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}aging} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{V}\PY{p}{)}
\PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}aging} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{LV}\PY{p}{)}
\PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious} \PY{o}{=} \PY{n}{parts}\PY{p}{(}\PY{n}{S\PYZus{}type}\PY{p}{,} \PY{o}{:}\PY{n}{LSV}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    \hypertarget{define-the-typed-infectious-disease-aggregate-population-system-structure-diagrams}{%
\subsubsection{Define the typed infectious disease aggregate population
system structure
diagrams}\label{define-the-typed-infectious-disease-aggregate-population-system-structure-diagrams}}

    \hypertarget{define-the-typed-seir-aggregate-population-system-structure-diagram}{%
\paragraph{Define the typed SEIR aggregate population system structure
diagram}\label{define-the-typed-seir-aggregate-population-system-structure-diagram}}

    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{22}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{c}{\PYZsh{} the id flow of each stock maps to the aging flow in the S\PYZus{}type daigram in this example}
\PY{n}{S\PYZus{}seir}\PY{o}{=}\PY{n}{StockAndFlowStructure}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{S}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{birth}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{incid}\PY{p}{,}\PY{o}{:}\PY{n}{deathS}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idS}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{E}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{incid}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}E}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{inf}\PY{p}{,}\PY{o}{:}\PY{n}{deathE}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}E}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}inf}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathE}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idE}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n+nb}{I}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{inf}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}I}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{rec}\PY{p}{,}\PY{o}{:}\PY{n}{deathI}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}I}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}rec}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idI}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{p}{,}\PY{o}{:}\PY{n}{NI}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{R}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{rec}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}R}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathR}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}R}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathR}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idR}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{birth}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birth}\PY{p}{,}\PY{o}{:}\PY{n}{incid}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,}\PY{o}{:}\PY{n}{inf}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}inf}\PY{p}{,}\PY{o}{:}\PY{n}{rec}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}rec}\PY{p}{,}\PY{o}{:}\PY{n}{deathS}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{p}{,}\PY{o}{:}\PY{n}{deathE}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathE}\PY{p}{,}\PY{o}{:}\PY{n}{deathI}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{p}{,}\PY{o}{:}\PY{n}{deathR}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathR}\PY{p}{,}
        \PY{o}{:}\PY{n}{id\PYZus{}S}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idS}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}E}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idE}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}I}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idI}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}R}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idR}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birth}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{,}\PY{o}{:}\PY{n}{NI}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}incid}\PY{p}{)}
\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    define the typed SEIR model, which is a ACSetTransformation mapped from
the S\_seir model to the S\_type model.

    \begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{juliaCodeAndExamples/s_seir.png}
\caption{stratifications.jpg}
\end{figure}


    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{23}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{t\PYZus{}seir}\PY{o}{=}\PY{n}{ACSetTransformation}\PY{p}{(}\PY{n}{S\PYZus{}seir}\PY{p}{,} \PY{n}{S\PYZus{}type}\PY{p}{,}
  \PY{n}{S} \PY{o}{=} \PY{p}{[}\PY{n}{s}\PY{p}{,} \PY{n}{s}\PY{p}{,} \PY{n}{s}\PY{p}{,} \PY{n}{s}\PY{p}{]}\PY{p}{,}
  \PY{n}{SV} \PY{o}{=} \PY{p}{[}\PY{n}{sv\PYZus{}N}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{]}\PY{p}{,}
  \PY{n}{LS} \PY{o}{=} \PY{p}{[}\PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{]}\PY{p}{,}   
  \PY{n}{F} \PY{o}{=} \PY{p}{[}\PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{]}\PY{p}{,}    
  \PY{n+nb}{I} \PY{o}{=} \PY{p}{[}\PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{]}\PY{p}{,} 
  \PY{n}{O} \PY{o}{=} \PY{p}{[}\PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{]}\PY{p}{,}
  \PY{n}{V} \PY{o}{=} \PY{p}{[}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{]}\PY{p}{,}
  \PY{n}{LV} \PY{o}{=} \PY{p}{[}\PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{]}\PY{p}{,}
  \PY{n}{LSV} \PY{o}{=} \PY{p}{[}\PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{]}\PY{p}{,}
  \PY{n}{Name} \PY{o}{=} \PY{n}{name} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{n+nb}{nothing}  
\PY{p}{)}

\PY{n+nd}{@assert} \PY{n}{is\PYZus{}natural}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{23}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_55_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{define-the-typed-sis-aggregate-population-system-structure-diagram}{%
\paragraph{Define the typed SIS aggregate population system structure
diagram}\label{define-the-typed-sis-aggregate-population-system-structure-diagram}}

\begin{figure}
\centering
\includegraphics[width=0.45\columnwidth]{juliaCodeAndExamples/s_sis.png}
\caption{stratifications.jpg}
\end{figure}

    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{24}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{S\PYZus{}sis}\PY{o}{=}\PY{n}{StockAndFlowStructure}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{S}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{births}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{p}{,}\PY{o}{:}\PY{n}{newRecovery}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathS}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectious}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idS}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{p}{)}\PY{p}{)}\PY{p}{,}
            \PY{o}{:}\PY{n+nb}{I}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{newInfectious}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}I}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathI}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}I}\PY{p}{,}\PY{o}{:}\PY{n}{newRecovery}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idI}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newRecovery}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{p}{,}\PY{o}{:}\PY{n}{NS}\PY{p}{,}\PY{o}{:}\PY{n}{NI}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{births}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}births}\PY{p}{,}\PY{o}{:}\PY{n}{deathS}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathS}\PY{p}{,}\PY{o}{:}\PY{n}{deathI}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathI}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectious}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{,}\PY{o}{:}\PY{n}{newRecovery}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newRecovery}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idS}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}I}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idI}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{o}{:}\PY{n}{NI}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{o}{:}\PY{n}{NS}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectious}\PY{p}{)}
    \PY{p}{)}

\PY{n}{t\PYZus{}sis}\PY{o}{=}\PY{n}{ACSetTransformation}\PY{p}{(}\PY{n}{S\PYZus{}sis}\PY{p}{,} \PY{n}{S\PYZus{}type}\PY{p}{,}
  \PY{n}{S} \PY{o}{=} \PY{p}{[}\PY{n}{s}\PY{p}{,} \PY{n}{s}\PY{p}{]}\PY{p}{,}
  \PY{n}{SV} \PY{o}{=} \PY{p}{[}\PY{n}{sv\PYZus{}N}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{]}\PY{p}{,}
  \PY{n}{LS} \PY{o}{=} \PY{p}{[}\PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{]}\PY{p}{,}   
  \PY{n}{F} \PY{o}{=} \PY{p}{[}\PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{]}\PY{p}{,}    
  \PY{n+nb}{I} \PY{o}{=} \PY{p}{[}\PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{]}\PY{p}{,} 
  \PY{n}{O} \PY{o}{=} \PY{p}{[}\PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,}
  \PY{n}{V} \PY{o}{=} \PY{p}{[}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{]}\PY{p}{,}
  \PY{n}{LV} \PY{o}{=} \PY{p}{[}\PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,}
  \PY{n}{LSV} \PY{o}{=} \PY{p}{[}\PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{]}\PY{p}{,}
  \PY{n}{Name} \PY{o}{=} \PY{n}{name} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{n+nb}{nothing}  
\PY{p}{)}

\PY{n+nd}{@assert} \PY{n}{is\PYZus{}natural}\PY{p}{(}\PY{n}{t\PYZus{}sis}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{t\PYZus{}sis}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{24}{}
    
    \begin{center}
    \adjustimage{max size={0.5\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_58_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \begin{figure}
\centering
\includegraphics[width=0.6\columnwidth]{juliaCodeAndExamples/age_strata.png}
\caption{stratifications.jpg}
\end{figure}

    

    \hypertarget{define-the-typed-strata-e.g.-age-system-structure-diagrams}{%
\subsubsection{Define the typed strata system structure
diagrams}\label{define-the-typed-strata-e.g.-age-system-structure-diagrams}}

    \hypertarget{define-the-aging-strata-system-structure-diagram-by-three-age-groups-child-adult-and-senior}{%
\paragraph{Define the aging strata system structure diagram by three age
groups: Child, Adult and
Senior}\label{define-the-aging-strata-system-structure-diagram-by-three-age-groups-child-adult-and-senior}}

    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{25}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{S\PYZus{}age\PYZus{}strata}\PY{o}{=}\PY{n}{StockAndFlowStructure}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{Child}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{births}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}C}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsChild}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{agingChild}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}C}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}agingChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}id\PYZus{}C}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}Child}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}Child}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{Adult}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{agingChild}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}A}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsAdult}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{agingAdult}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}A}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}agingAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}id\PYZus{}A}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}Adult}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}Adult}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{Senior}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{agingAdult}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousSenior}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsSenior}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousSenior}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsSenior}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}id\PYZus{}S}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}Senior}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}Senior}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{births}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}births}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousChild}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousAdult}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousSenior}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{,}
        \PY{o}{:}\PY{n}{id\PYZus{}C}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}id\PYZus{}C}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}A}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}id\PYZus{}A}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}S}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}id\PYZus{}S}\PY{p}{,}
        \PY{o}{:}\PY{n}{agingChild}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}agingChild}\PY{p}{,}\PY{o}{:}\PY{n}{agingAdult}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}agingAdult}\PY{p}{,}
        \PY{o}{:}\PY{n}{deathsChild}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsChild}\PY{p}{,}\PY{o}{:}\PY{n}{deathsAdult}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsAdult}\PY{p}{,}\PY{o}{:}\PY{n}{deathsSenior}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsSenior}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{o}{:}\PY{n}{NI\PYZus{}Child}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}Child}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{)}\PY{p}{,}
                  \PY{o}{:}\PY{n}{NI\PYZus{}Adult}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}Adult}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{)}\PY{p}{,}
                  \PY{o}{:}\PY{n}{NI\PYZus{}Senior}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}Senior}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousChild}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousAdult}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousSenior}\PY{p}{)}\PY{p}{)}
\PY{p}{)}

\PY{n}{t\PYZus{}age\PYZus{}strata}\PY{o}{=}\PY{n}{ACSetTransformation}\PY{p}{(}\PY{n}{S\PYZus{}age\PYZus{}strata}\PY{p}{,} \PY{n}{S\PYZus{}type}\PY{p}{,}
  \PY{n}{S} \PY{o}{=} \PY{p}{[}\PY{n}{s}\PY{p}{,}\PY{n}{s}\PY{p}{,}\PY{n}{s}\PY{p}{]}\PY{p}{,}
  \PY{n}{SV} \PY{o}{=} \PY{p}{[}\PY{n}{sv\PYZus{}N}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{]}\PY{p}{,}
  \PY{n}{LS} \PY{o}{=} \PY{p}{[}\PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{]}\PY{p}{,}     
  \PY{n}{F} \PY{o}{=} \PY{p}{[}\PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{]}\PY{p}{,}      
  \PY{n+nb}{I} \PY{o}{=} \PY{p}{[}\PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,} 
  \PY{n}{O} \PY{o}{=} \PY{p}{[}\PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,}
  \PY{n}{V} \PY{o}{=} \PY{p}{[}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{]}\PY{p}{,}      
  \PY{n}{LV} \PY{o}{=} \PY{p}{[}\PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,}
  \PY{n}{LSV} \PY{o}{=} \PY{p}{[}\PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{]}\PY{p}{,}
  \PY{n}{Name} \PY{o}{=} \PY{n}{name} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{n+nb}{nothing}  
\PY{p}{)}

\PY{n+nd}{@assert} \PY{n}{is\PYZus{}natural}\PY{p}{(}\PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{25}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_62_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}

    \begin{figure}
\centering
\includegraphics[width=0.6\columnwidth]{juliaCodeAndExamples/sex_strata.png}
\caption{stratifications.jpg}
\end{figure}


    \hypertarget{define-the-sex-strata-system-structure-diagram-by-two-sub-groups-female-and-male}{%
\paragraph{Define the sex strata system structure diagram by two
sub-groups: Female and
Male}\label{define-the-sex-strata-system-structure-diagram-by-two-sub-groups-female-and-male}}

    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{26}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{S\PYZus{}sex\PYZus{}strata}\PY{o}{=}\PY{n}{StockAndFlowStructure}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{F}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{birthsF}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}F}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsF}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}F}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idF}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}F}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}F}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{M}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{birthsM}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}M}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsM}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}M}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsM}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idM}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}M}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}M}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{birthsF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birthsF}\PY{p}{,}\PY{o}{:}\PY{n}{birthsM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birthsM}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}F}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idF}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}M}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idM}\PY{p}{,}
        \PY{o}{:}\PY{n}{deathsF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsF}\PY{p}{,}\PY{o}{:}\PY{n}{deathsM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsM}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}birthsF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}birthsM}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NI\PYZus{}F}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}F}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{,}
                  \PY{o}{:}\PY{n}{NI\PYZus{}M}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}M}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{)}
\PY{p}{)}

\PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{o}{=}\PY{n}{ACSetTransformation}\PY{p}{(}\PY{n}{S\PYZus{}sex\PYZus{}strata}\PY{p}{,} \PY{n}{S\PYZus{}type}\PY{p}{,}
  \PY{n}{S} \PY{o}{=} \PY{p}{[}\PY{n}{s}\PY{p}{,}\PY{n}{s}\PY{p}{]}\PY{p}{,}
  \PY{n}{SV} \PY{o}{=} \PY{p}{[}\PY{n}{sv\PYZus{}N}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{]}\PY{p}{,}
  \PY{n}{LS} \PY{o}{=} \PY{p}{[}\PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{]}\PY{p}{,}     
  \PY{n}{F} \PY{o}{=} \PY{p}{[}\PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{]}\PY{p}{,}      
  \PY{n+nb}{I} \PY{o}{=} \PY{p}{[}\PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,} 
  \PY{n}{O} \PY{o}{=} \PY{p}{[}\PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,}
  \PY{n}{V} \PY{o}{=} \PY{p}{[}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{]}\PY{p}{,}      
  \PY{n}{LV} \PY{o}{=} \PY{p}{[}\PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{]}\PY{p}{,}
  \PY{n}{LSV} \PY{o}{=} \PY{p}{[}\PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{]}\PY{p}{,}
  \PY{n}{Name} \PY{o}{=} \PY{n}{name} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{n+nb}{nothing}  
\PY{p}{)}

\PY{n+nd}{@assert} \PY{n}{is\PYZus{}natural}\PY{p}{(}\PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{26}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_65_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{build-the-stratification-models}{%
\subsubsection{Build the stratification
models}\label{build-the-stratification-models}}

    \hypertarget{build-the-age-stratification-models}{%
\paragraph{Build the Age stratification
models}\label{build-the-age-stratification-models}}

    The SEIR age stratified model:

    \begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{juliaCodeAndExamples/seir_age.png}
\caption{stratifications.jpg}
\end{figure}
    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{27}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seir\PYZus{}age} \PY{o}{=} \PY{n}{stratify}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{,} \PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{typed\PYZus{}stratify}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{,} \PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{27}{}
    
    \begin{center}
    \adjustimage{max size={0.9\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_70_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    The SIS age stratified model:

    \begin{figure}
\centering
\includegraphics[width=0.7\columnwidth]{juliaCodeAndExamples/sis_age.png}
\caption{stratifications.jpg}
\end{figure}
    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{28}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{sis\PYZus{}age} \PY{o}{=} \PY{n}{stratify}\PY{p}{(}\PY{n}{t\PYZus{}sis}\PY{p}{,} \PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{typed\PYZus{}stratify}\PY{p}{(}\PY{n}{t\PYZus{}sis}\PY{p}{,} \PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{28}{}
    
    \begin{center}
    \adjustimage{max size={0.8\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_73_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{build-the-sex-stratification-models}{%
\paragraph{Build the Sex stratification
models}\label{build-the-sex-stratification-models}}

    The SEIR sex stratified model:

     \begin{figure}
\centering
\includegraphics[width=0.6\columnwidth]{juliaCodeAndExamples/seir_sex.png}
\caption{stratifications.jpg}
\end{figure}
   

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{29}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seir\PYZus{}sex} \PY{o}{=} \PY{n}{stratify}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{,} \PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{p}{)}\PY{p}{;}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{typed\PYZus{}stratify}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{,} \PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{p}{)}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{29}{}
    
    \begin{center}
    \adjustimage{max size={0.8\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_77_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    The SIS sex stratified model:

    \begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{juliaCodeAndExamples/sis_sex.png}
\caption{stratifications.jpg}
\end{figure}
    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{30}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{sis\PYZus{}sex} \PY{o}{=} \PY{n}{stratify}\PY{p}{(}\PY{n}{t\PYZus{}sis}\PY{p}{,} \PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{p}{)}\PY{p}{;}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{typed\PYZus{}stratify}\PY{p}{(}\PY{n}{t\PYZus{}sis}\PY{p}{,} \PY{n}{t\PYZus{}sex\PYZus{}strata}\PY{p}{)}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{30}{}
    
    \begin{center}
    \adjustimage{max size={0.8\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_80_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{build-the-stratified-model-with-multiple-stratas-e.g.-both-age-and-sex-stratas}{%
\subsection{Build the stratified model with multiple stratas (e.g., both
age and sex
stratas)}\label{build-the-stratified-model-with-multiple-stratas-e.g.-both-age-and-sex-stratas}}

    We can build the stratified model with multiple dimensions (e.g., by age
and sex) by calculating the pullback of the diseease model and multiple
strata models. We create an example to stratify the SEIR model by both
sex and age dimensions in this project. It is notable that when combine
multiple strata model together to calculate the pullback, we may need to
add some extra components to the strata models to accomodate to the
other strata models. For example, we need to add an id flow of aging of
each stock to the sex strata model to keep the aging flows in the
stratified results.

    

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{31}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{S\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{o}{=}\PY{n}{StockAndFlowStructure}\PY{p}{(}
    \PY{p}{(}\PY{o}{:}\PY{n}{F}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{birthsF}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}F}\PY{p}{,}\PY{o}{:}\PY{n}{agingF}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsF}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}F}\PY{p}{,}\PY{o}{:}\PY{n}{agingF}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}agingF}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}F}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}F}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{,}
        \PY{o}{:}\PY{n}{M}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{p}{(}\PY{o}{:}\PY{n}{birthsM}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}M}\PY{p}{,}\PY{o}{:}\PY{n}{agingM}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{deathsM}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}M}\PY{p}{,}\PY{o}{:}\PY{n}{agingM}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}deathsM}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}idM}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}agingM}\PY{p}{)}\PY{p}{,}\PY{p}{(}\PY{o}{:}\PY{n}{NI\PYZus{}M}\PY{p}{,}\PY{o}{:}\PY{n}{NS\PYZus{}M}\PY{p}{,}\PY{o}{:}\PY{n}{N}\PY{p}{)}\PY{p}{)}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{birthsF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birthsF}\PY{p}{,}\PY{o}{:}\PY{n}{birthsM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}birthsM}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{newInfectiousM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}F}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idF}\PY{p}{,}\PY{o}{:}\PY{n}{id\PYZus{}M}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}idM}\PY{p}{,}
        \PY{o}{:}\PY{n}{deathsF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsF}\PY{p}{,}\PY{o}{:}\PY{n}{deathsM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}deathsM}\PY{p}{,}\PY{o}{:}\PY{n}{agingF}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}agingF}\PY{p}{,}\PY{o}{:}\PY{n}{agingM}\PY{o}{=\PYZgt{}}\PY{o}{:}\PY{n}{v\PYZus{}agingM}\PY{p}{)}\PY{p}{,}
    \PY{p}{(}\PY{o}{:}\PY{n}{N}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}birthsF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}birthsM}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NI\PYZus{}F}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}F}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{,}
                  \PY{o}{:}\PY{n}{NI\PYZus{}M}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{,} \PY{o}{:}\PY{n}{NS\PYZus{}M}\PY{o}{=\PYZgt{}}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousF}\PY{p}{,}\PY{o}{:}\PY{n}{v\PYZus{}newInfectiousM}\PY{p}{)}\PY{p}{)}
\PY{p}{)}

\PY{n}{t\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{o}{=}\PY{n}{ACSetTransformation}\PY{p}{(}\PY{n}{S\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{p}{,} \PY{n}{S\PYZus{}type}\PY{p}{,}
  \PY{n}{S} \PY{o}{=} \PY{p}{[}\PY{n}{s}\PY{p}{,}\PY{n}{s}\PY{p}{]}\PY{p}{,}
  \PY{n}{SV} \PY{o}{=} \PY{p}{[}\PY{n}{sv\PYZus{}N}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{,} \PY{n}{sv\PYZus{}NI}\PY{p}{,} \PY{n}{sv\PYZus{}NS}\PY{p}{]}\PY{p}{,}
  \PY{n}{LS} \PY{o}{=} \PY{p}{[}\PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{,} \PY{n}{lsn\PYZus{}NI}\PY{p}{,} \PY{n}{lsn\PYZus{}NS}\PY{p}{,} \PY{n}{lsn\PYZus{}N}\PY{p}{]}\PY{p}{,}     
  \PY{n}{F} \PY{o}{=} \PY{p}{[}\PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}births}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}newInfectious}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}deaths}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{,} \PY{n}{f\PYZus{}aging}\PY{p}{]}\PY{p}{,}      
  \PY{n+nb}{I} \PY{o}{=} \PY{p}{[}\PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{,} \PY{n}{i\PYZus{}births}\PY{p}{,} \PY{n}{i\PYZus{}newInfectious}\PY{p}{,} \PY{n}{i\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{i\PYZus{}aging}\PY{p}{]}\PY{p}{,} 
  \PY{n}{O} \PY{o}{=} \PY{p}{[}\PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{,} \PY{n}{o\PYZus{}deaths}\PY{p}{,} \PY{n}{o\PYZus{}newInfectious}\PY{p}{,} \PY{n}{o\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{o\PYZus{}aging}\PY{p}{]}\PY{p}{,}
  \PY{n}{V} \PY{o}{=} \PY{p}{[}\PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}births}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}newInfectious}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}deaths}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{,} \PY{n}{v\PYZus{}aging}\PY{p}{]}\PY{p}{,}      
  \PY{n}{LV} \PY{o}{=} \PY{p}{[}\PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{,} \PY{n}{lv\PYZus{}deaths}\PY{p}{,} \PY{n}{lv\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lv\PYZus{}firstOrderDelay}\PY{p}{,} \PY{n}{lv\PYZus{}aging}\PY{p}{]}\PY{p}{,}
  \PY{n}{LSV} \PY{o}{=} \PY{p}{[}\PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}N\PYZus{}births}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NI\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{,} \PY{n}{lsv\PYZus{}NS\PYZus{}newInfectious}\PY{p}{]}\PY{p}{,}
  \PY{n}{Name} \PY{o}{=} \PY{n}{name} \PY{o}{\PYZhy{}}\PY{o}{\PYZgt{}} \PY{n+nb}{nothing}  
\PY{p}{)}

\PY{n+nd}{@assert} \PY{n}{is\PYZus{}natural}\PY{p}{(}\PY{n}{t\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{t\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{31}{}
    
    \begin{center}
    \adjustimage{max size={0.6\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_84_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \begin{figure}
\centering
\includegraphics{juliaCodeAndExamples/seir_age_sex.png}
\caption{seir\_age\_sex.png}
\end{figure}

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{32}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{seir\PYZus{}sex\PYZus{}age} \PY{o}{=} \PY{n}{stratify}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{,} \PY{n}{t\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{p}{,} \PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}
\PY{n}{Graph\PYZus{}typed}\PY{p}{(}\PY{n}{typed\PYZus{}stratify}\PY{p}{(}\PY{n}{t\PYZus{}seir}\PY{p}{,} \PY{n}{t\PYZus{}sex\PYZus{}strata\PYZus{}withAge}\PY{p}{,} \PY{n}{t\PYZus{}age\PYZus{}strata}\PY{p}{)}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{32}{}
    
    \begin{center}
    \adjustimage{max size={0.9\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_86_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    

    \hypertarget{solve-the-stratified-model}{%
\subsection{Solve the stratified
model}\label{solve-the-stratified-model}}

    We can assign the functions to the auxiliary variables and convert the
stratified system structure diagrams to the stock \& flow diagrams.
Then, we can map the stock \& flow diagrams to the ODEs, and solve it.

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{33}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{sis\PYZus{}sex\PYZus{}flatten}\PY{o}{=}\PY{n}{rebuildSystemStructureByFlattenSymbols}\PY{p}{(}\PY{n}{sis\PYZus{}sex}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    Define the functions of each auxiliary variable, and map to stock \&
flow diagram:

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{34}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{f\PYZus{}birthF}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{p}\PY{o}{.}\PY{n}{μF}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{NN}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}
\PY{n}{f\PYZus{}birthM}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{p}\PY{o}{.}\PY{n}{μM}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{NN}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}

\PY{n}{f\PYZus{}infF}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=} \PY{n}{p}\PY{o}{.}\PY{n}{βF}\PY{o}{*}\PY{n}{u}\PY{o}{.}\PY{n}{SF}\PY{o}{*}\PY{p}{(}\PY{n}{p}\PY{o}{.}\PY{n}{ff}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{NINI\PYZus{}F}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{/}\PY{n}{uN}\PY{o}{.}\PY{n}{NSNS\PYZus{}F}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{+}\PY{n}{p}\PY{o}{.}\PY{n}{fm}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{NINI\PYZus{}M}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{/}\PY{n}{uN}\PY{o}{.}\PY{n}{NSNS\PYZus{}M}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{p}{)}
\PY{n}{f\PYZus{}infM}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=} \PY{n}{p}\PY{o}{.}\PY{n}{βM}\PY{o}{*}\PY{n}{u}\PY{o}{.}\PY{n}{SM}\PY{o}{*}\PY{p}{(}\PY{n}{p}\PY{o}{.}\PY{n}{mf}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{NINI\PYZus{}F}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{/}\PY{n}{uN}\PY{o}{.}\PY{n}{NSNS\PYZus{}F}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{+}\PY{n}{p}\PY{o}{.}\PY{n}{mm}\PY{o}{*}\PY{n}{uN}\PY{o}{.}\PY{n}{NINI\PYZus{}M}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{/}\PY{n}{uN}\PY{o}{.}\PY{n}{NSNS\PYZus{}M}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{p}{)}

\PY{n}{f\PYZus{}recF}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{IF}\PY{o}{/}\PY{n}{p}\PY{o}{.}\PY{n}{trecoveryF}
\PY{n}{f\PYZus{}recM}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{IM}\PY{o}{/}\PY{n}{p}\PY{o}{.}\PY{n}{trecoveryM}

\PY{n}{f\PYZus{}deathSF}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{SF}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δF}
\PY{n}{f\PYZus{}deathIF}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{IF}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δF}
\PY{n}{f\PYZus{}deathSM}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{SM}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δM}
\PY{n}{f\PYZus{}deathIM}\PY{p}{(}\PY{n}{u}\PY{p}{,}\PY{n}{uN}\PY{p}{,}\PY{n}{p}\PY{p}{,}\PY{n}{t}\PY{p}{)}\PY{o}{=}\PY{n}{u}\PY{o}{.}\PY{n}{IM}\PY{o}{*}\PY{n}{p}\PY{o}{.}\PY{n}{δM}

\PY{n}{v\PYZus{}sis\PYZus{}sex}\PY{o}{=}\PY{p}{(}\PY{o}{:}\PY{n}{v\PYZus{}birthsv\PYZus{}birthsF}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}birthF}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}birthsv\PYZus{}birthsM}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}birthM}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}newInfectiousv\PYZus{}newInfectiousF}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}infF}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}newInfectiousv\PYZus{}newInfectiousM}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}infM}\PY{p}{,}
\PY{o}{:}\PY{n}{v\PYZus{}newRecoveryv\PYZus{}idF}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}recF}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}newRecoveryv\PYZus{}idM}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}recM}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}deathSv\PYZus{}deathsF}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathSF}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}deathIv\PYZus{}deathsF}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathIF}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}deathSv\PYZus{}deathsM}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathSM}\PY{p}{,} \PY{o}{:}\PY{n}{v\PYZus{}deathIv\PYZus{}deathsM}\PY{o}{=\PYZgt{}}\PY{n}{f\PYZus{}deathIM}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    Convert the system structure diagram to the stock \& flow diagram:

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{35}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{sis\PYZus{}sex\PYZus{}SF}\PY{o}{=}\PY{n}{convertSystemStructureToStockFlow}\PY{p}{(}\PY{n}{sis\PYZus{}sex\PYZus{}flatten}\PY{p}{,}\PY{n}{v\PYZus{}sis\PYZus{}sex}\PY{p}{)}\PY{p}{;}
\end{Verbatim}
\end{tcolorbox}

    Solve the ODEs of the converted stock \& flow diagram:

    \begin{tcolorbox}[breakable, size=fbox, boxrule=1pt, pad at break*=1mm,colback=cellbackground, colframe=cellborder]
\prompt{In}{incolor}{36}{\boxspacing}
\begin{Verbatim}[commandchars=\\\{\}]
\PY{n}{p\PYZus{}sis\PYZus{}sex} \PY{o}{=} \PY{n}{LVector}\PY{p}{(}
    \PY{n}{βF}\PY{o}{=}\PY{l+m+mf}{0.5}\PY{p}{,} \PY{n}{βM}\PY{o}{=}\PY{l+m+mf}{0.6}\PY{p}{,} \PY{n}{μM}\PY{o}{=}\PY{l+m+mi}{0}\PY{p}{,} \PY{n}{μF}\PY{o}{=}\PY{l+m+mf}{0.03}\PY{o}{/}\PY{l+m+mi}{365}\PY{o}{/}\PY{l+m+mf}{2.0}\PY{p}{,} \PY{n}{δM}\PY{o}{=}\PY{l+m+mf}{0.05}\PY{o}{/}\PY{l+m+mi}{365}\PY{o}{/}\PY{l+m+mf}{2.0}\PY{p}{,} \PY{n}{δF}\PY{o}{=}\PY{l+m+mf}{0.01}\PY{o}{/}\PY{l+m+mi}{365}\PY{o}{/}\PY{l+m+mf}{2.0}\PY{p}{,} \PY{n}{trecoveryM}\PY{o}{=}\PY{l+m+mf}{5.0}\PY{p}{,} \PY{n}{trecoveryF}\PY{o}{=}\PY{l+m+mf}{5.0}\PY{p}{,}
    \PY{n}{ff}\PY{o}{=}\PY{l+m+mf}{0.5}\PY{p}{,} \PY{n}{fm}\PY{o}{=}\PY{l+m+mf}{0.5}\PY{p}{,} \PY{n}{mf}\PY{o}{=}\PY{l+m+mf}{0.5}\PY{p}{,} \PY{n}{mm}\PY{o}{=}\PY{l+m+mf}{0.5}
\PY{p}{)}
\PY{n}{u0\PYZus{}sis\PYZus{}sex} \PY{o}{=} \PY{n}{LVector}\PY{p}{(}
    \PY{n}{SM}\PY{o}{=}\PY{l+m+mf}{5400.0}\PY{p}{,} \PY{n}{SF}\PY{o}{=}\PY{l+m+mf}{4600.0}\PY{p}{,} \PY{n}{IM}\PY{o}{=}\PY{l+m+mf}{10.0}\PY{p}{,} \PY{n}{IF}\PY{o}{=}\PY{l+m+mf}{1.0}
\PY{p}{)}

\PY{n}{prob\PYZus{}sis\PYZus{}sex} \PY{o}{=} \PY{n}{ODEProblem}\PY{p}{(}\PY{n}{vectorfield}\PY{p}{(}\PY{n}{sis\PYZus{}sex\PYZus{}SF}\PY{p}{)}\PY{p}{,}\PY{n}{u0\PYZus{}sis\PYZus{}sex}\PY{p}{,}\PY{p}{(}\PY{l+m+mf}{0.0}\PY{p}{,}\PY{l+m+mf}{50.0}\PY{p}{)}\PY{p}{,}\PY{n}{p\PYZus{}sis\PYZus{}sex}\PY{p}{)}\PY{p}{;}
\PY{n}{sol\PYZus{}sis\PYZus{}sex} \PY{o}{=} \PY{n}{solve}\PY{p}{(}\PY{n}{prob\PYZus{}sis\PYZus{}sex}\PY{p}{,}\PY{n}{Tsit5}\PY{p}{(}\PY{p}{)}\PY{p}{,}\PY{n}{abstol}\PY{o}{=}\PY{l+m+mf}{1e\PYZhy{}8}\PY{p}{)}\PY{p}{;}
\PY{n}{plot}\PY{p}{(}\PY{n}{sol\PYZus{}sis\PYZus{}sex}\PY{p}{)}
\end{Verbatim}
\end{tcolorbox}
 
            
\prompt{Out}{outcolor}{36}{}
    
    \begin{center}
    \adjustimage{max size={0.42\linewidth}{0.9\paperheight}}{juliaCodeAndExamples/output_95_0.pdf}
    \end{center}
    { \hspace*{\fill} \\}
    
    % Add a bibliography block to the postdoc
%\end{document}


==> preamble1.tex <==
\usepackage{amssymb,mathrsfs,amsmath,amsfonts,graphicx,pdfpages,todonotes,bbold,float}
\usepackage{caption}
\usepackage{subcaption}

% Julia code
%\usepackage{minted}

% Quiver
%\usepackage{quiver}


% colors
\usepackage{xcolor}
\usepackage{framed,color}

\definecolor{shadecolor}{rgb}{1,0.8,0.3}
\definecolor{myurlcolor}{rgb}{0.5,0,0}
\definecolor{mycitecolor}{rgb}{0,0,0.7}
\definecolor{myrefcolor}{rgb}{0,0,0.7}
\definecolor{hyperrefcolor}{rgb}{0.5,0,0}

% hyperlinks

\usepackage{hyperref}
\hypersetup{
	colorlinks,
	linkcolor={hyperrefcolor},
	citecolor={mycitecolor},
	urlcolor={hyperrefcolor}
}


%\usepackage[clean]{svg}

% font for definitions 

\newcommand{\define}[1]{{\bf \boldmath{#1}}}

% call proofs "proof sketch"

\renewcommand*{\proofname}{Proof Sketch}

% sets

\newcommand{\namedset}[1]{\mathbb{#1}}
\newcommand{\R}{\namedset{R}}
\newcommand{\Naturals}{\namedset{N}}
\newcommand{\Integers}{\namedset{Z}}

% categories

\newcommand{\namedcat}[1]{\mathsf{#1}}
\newcommand{\Set}{\namedcat{Set}}
\newcommand{\Fin}{\namedcat{Fin}}
\newcommand{\Graph}{\namedcat{Graph}}
\newcommand{\C}{\namedcat{C}}
\newcommand{\G}{\namedcat{G}}
\renewcommand{\H}{\namedcat{H}}
\newcommand{\K}{\namedcat{K}}
\newcommand{\Cat}{\namedcat{Cat}}
\newcommand{\CMC}{\namedcat{CMC}}
\newcommand{\CMon}{\namedcat{CMon}}
\newcommand{\Petri}{\namedcat{Petri}}
\newcommand{\cPetri}{\namedcat{cPetri}}
\newcommand{\Dynam}{\namedcat{Dynam}}
\newcommand{\StockFlow}{\namedcat{StockFlow}}
\newcommand{\CausalLoop}{\namedcat{CausalLoop}}
\newcommand{\SystemStructure}{\namedcat{SystemStructure}}
\newcommand{\Open}{\namedcat{Open}}

\newcommand{\4}{\mathbf{4}}
\newcommand{\8}{\mathbf{8}}

\newcommand{\X}{\namedcat{X}}
\newcommand{\A}{\namedcat{A}}

\newcommand{\id}[1]{\mathbb{1}_{#1}}
\newcommand{\compose}{\circ}
\newcommand{\dialspan}{\namedcat{DialSpan}(\namedcat{B},\namedcat{C})}
\newcommand{\product}{\&}
\newcommand{\coproduct}{\oplus}
\newcommand{\productmap}[2]{\langle #1, #2 \rangle}
\newcommand{\coproductmap}[2]{[#1,#2]}
\newcommand{\tensor}{\oslash}

\newcommand{\PSet}{\Set_{\perp}}
\newcommand{\UNFOLD}{\mathtt{UNFOLD}}
\newcommand{\Net}[1]{#1\text{-}\mathsf{Net}}
\newcommand{\Adj}{\mathbb{A}\mathsf{dj}}
\newcommand{\Csp}{\mathbb{C}\mathsf{sp}}
\newcommand{\Hom}{\mathrm{Hom}}
\newcommand{\p}{\mathrm{p}}
%\renewcommand{\r}{\mathrm{r}}
\newcommand{\ff}{f}

% schema for stock-flow diagrams
\newcommand{\stock}{\mathrm{stock}}
\newcommand{\flow}{\mathrm{flow}}
\newcommand{\link}{\mathrm{link}}
\newcommand{\variable}{\mathrm{variable}}
\newcommand{\sumvariable}{\mathrm{sum variable}}
\newcommand{\sumlink}{\mathrm{sum link}}

\renewcommand{\S}{\mathrm{S}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\V}{\mathrm{V}}
\newcommand{\SV}{\mathrm{SV}}
\renewcommand{\I}{\mathrm{I}}
\renewcommand{\O}{\mathrm{O}}
\newcommand{\LS}{\mathrm{LS}}
\newcommand{\LV}{\mathrm{LV}}
\newcommand{\LSV}{\mathrm{LSV}}

\newcommand{\is}{\mathrm{is}}
\newcommand{\ifn}{\mathrm{ifn}}
\newcommand{\os}{\mathrm{os}}
\newcommand{\ofn}{\mathrm{ofn}}
\newcommand{\lss}{\mathrm{lss}}
\newcommand{\lssv}{\mathrm{lssv}}
\newcommand{\lsvv}{\mathrm{lsvv}}
\newcommand{\fv}{\mathrm{fv}}
\newcommand{\lvs}{\mathrm{lvs}}
\newcommand{\lvv}{\mathrm{lvv}}
\newcommand{\lsvsv}{\mathrm{lsvsv}}

% schema for causal loop diagrams
\newcommand{\CL}{\mathrm{CL}}
\renewcommand{\E}{\mathrm{E}}
\newcommand{\Node}{\mathrm{N}}

% sum variables for stratified model:

\newcommand{\N}{\mathrm{N}}
\newcommand{\NS}{\mathrm{NS}}
\newcommand{\NI}{\mathrm{NI}}

% subscripts
\newcommand{\ICU}{\mathrm{ICU}}
\newcommand{\NICU}{\mathrm{NICU}}

\makeatletter
\newcommand*{\relrelbarsep}{.386ex}
\newcommand*{\relrelbar}{%
  \mathrel{%
    \mathpalette\@relrelbar\relrelbarsep
  }%
}
\newcommand*{\@relrelbar}[2]{%
  \raise#2\hbox to 0pt{$\m@th#1\relbar$\hss}%
  \lower#2\hbox{$\m@th#1\relbar$}%
}
\providecommand*{\rightrightarrowsfill@}{%
  \arrowfill@\relrelbar\relrelbar\rightrightarrows
}
\providecommand*{\leftleftarrowsfill@}{%
  \arrowfill@\leftleftarrows\relrelbar\relrelbar
}
\providecommand*{\xrightrightarrows}[2][]{%
  \ext@arrow 0359\rightrightarrowsfill@{#1}{#2}%
}
\providecommand*{\xleftleftarrows}[2][]{%
  \ext@arrow 3095\leftleftarrowsfill@{#1}{#2}%
}
\makeatother

\usepackage{enumerate}

\newcommand{\maps}{\colon}


%%%%%% preamble for the appendix %%%%%%
%\documentclass[5pt]{article}
%\documentclass[graybox]{svmult}

    \usepackage[breakable]{tcolorbox}
    \usepackage{parskip} % Stop auto-indenting (to mimic markdown behaviour)
    
    \usepackage{iftex}
    \ifPDFTeX
    	\usepackage[T1]{fontenc}
    	\usepackage{mathpazo}
    \else
    	\usepackage{fontspec}
    \fi
    \DeclareUnicodeCharacter{03BC}{$\mu$}
    \DeclareUnicodeCharacter{03B2}{$\beta$}
    \DeclareUnicodeCharacter{03B4}{$\delta$}
    \DeclareUnicodeCharacter{03B1}{$\alpha$}
    % Basic figure setup, for now with no caption control since it's done
    % automatically by Pandoc (which extracts ![](path) syntax from Markdown).
    \usepackage{graphicx}
    % Maintain compatibility with old templates. Remove in nbconvert 6.0
    \let\Oldincludegraphics\includegraphics
    % Ensure that by default, figures have no caption (until we provide a
    % proper Figure object with a Caption API and a way to capture that
    % in the conversion process - todo).
    \usepackage{caption}
    \DeclareCaptionFormat{nocaption}{}
    \captionsetup{format=nocaption,aboveskip=0pt,belowskip=0pt}

    \usepackage[Export]{adjustbox} % Used to constrain images to a maximum size
    \adjustboxset{max size={0.9\linewidth}{0.9\paperheight}}
    \usepackage{float}
    \floatplacement{figure}{H} % forces figures to be placed at the correct location

    % Hack from http://tex.stackexchange.com/a/47451/13684:
    \AtBeginDocument{%
        \def\PYZsq{\textquotesingle}% Upright quotes in Pygmentized code
    }
    
    
    
    % package upquote cause the error message of "LaTeX Error: Option clash for package textcomp."
    \usepackage{upquote} % Upright quotes for verbatim code
    \usepackage{eurosym} % defines \euro
    \usepackage[mathletters]{ucs} % Extended unicode (utf-8) support
    \usepackage{fancyvrb} % verbatim replacement that allows latex
    \usepackage{grffile} % extends the file name processing of package graphics 
                         % to support a larger range
    \makeatletter % fix for grffile with XeLaTeX

    \makeatother

    % The hyperref package gives us a pdf with properly built
    % internal navigation ('pdf bookmarks' for the table of contents,
    % internal cross-reference links, web links for URLs, etc.)

    % The default LaTeX title has an obnoxious amount of whitespace. By default,
    % titling removes some of it. It also provides customization options.

    \usepackage{longtable} % longtable support required by pandoc >1.10
    \usepackage{booktabs}  % table support for pandoc > 1.12.2
    \usepackage[inline]{enumitem} % IRkernel/repr support (it uses the enumerate* environment)
    \usepackage[normalem]{ulem} % ulem is needed to support strikethroughs (\sout)
                                % normalem makes italics be italics, not underlines

    

    
    % Colors for the hyperref package
    \definecolor{urlcolor}{rgb}{0,.145,.698}
    \definecolor{linkcolor}{rgb}{.71,0.21,0.01}
    \definecolor{citecolor}{rgb}{.12,.54,.11}

    % ANSI colors
    \definecolor{ansi-black}{HTML}{3E424D}
    \definecolor{ansi-black-intense}{HTML}{282C36}
    \definecolor{ansi-red}{HTML}{E75C58}
    \definecolor{ansi-red-intense}{HTML}{B22B31}
    \definecolor{ansi-green}{HTML}{00A250}
    \definecolor{ansi-green-intense}{HTML}{007427}
    \definecolor{ansi-yellow}{HTML}{DDB62B}
    \definecolor{ansi-yellow-intense}{HTML}{B27D12}
    \definecolor{ansi-blue}{HTML}{208FFB}
    \definecolor{ansi-blue-intense}{HTML}{0065CA}
    \definecolor{ansi-magenta}{HTML}{D160C4}
    \definecolor{ansi-magenta-intense}{HTML}{A03196}
    \definecolor{ansi-cyan}{HTML}{60C6C8}
    \definecolor{ansi-cyan-intense}{HTML}{258F8F}
    \definecolor{ansi-white}{HTML}{C5C1B4}
    \definecolor{ansi-white-intense}{HTML}{A1A6B2}
    \definecolor{ansi-default-inverse-fg}{HTML}{FFFFFF}
    \definecolor{ansi-default-inverse-bg}{HTML}{000000}

    % commands and environments needed by pandoc snippets
    % extracted from the output of `pandoc -s`
    \providecommand{\tightlist}{%
      \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}
    \DefineVerbatimEnvironment{Highlighting}{Verbatim}{commandchars=\\\{\}}
    % Add ',fontsize=\small' for more characters per line
    \newenvironment{Shaded}{}{}
    \newcommand{\KeywordTok}[1]{\textcolor[rgb]{0.00,0.44,0.13}{\textbf{{#1}}}}
    \newcommand{\DataTypeTok}[1]{\textcolor[rgb]{0.56,0.13,0.00}{{#1}}}
    \newcommand{\DecValTok}[1]{\textcolor[rgb]{0.25,0.63,0.44}{{#1}}}
    \newcommand{\BaseNTok}[1]{\textcolor[rgb]{0.25,0.63,0.44}{{#1}}}
    \newcommand{\FloatTok}[1]{\textcolor[rgb]{0.25,0.63,0.44}{{#1}}}
    \newcommand{\CharTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\StringTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\CommentTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textit{{#1}}}}
    \newcommand{\OtherTok}[1]{\textcolor[rgb]{0.00,0.44,0.13}{{#1}}}
    \newcommand{\AlertTok}[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{{#1}}}}
    \newcommand{\FunctionTok}[1]{\textcolor[rgb]{0.02,0.16,0.49}{{#1}}}
    \newcommand{\RegionMarkerTok}[1]{{#1}}
    \newcommand{\ErrorTok}[1]{\textcolor[rgb]{1.00,0.00,0.00}{\textbf{{#1}}}}
    \newcommand{\NormalTok}[1]{{#1}}
    
    % Additional commands for more recent versions of Pandoc
    \newcommand{\ConstantTok}[1]{\textcolor[rgb]{0.53,0.00,0.00}{{#1}}}
    \newcommand{\SpecialCharTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\VerbatimStringTok}[1]{\textcolor[rgb]{0.25,0.44,0.63}{{#1}}}
    \newcommand{\SpecialStringTok}[1]{\textcolor[rgb]{0.73,0.40,0.53}{{#1}}}
    \newcommand{\ImportTok}[1]{{#1}}
    \newcommand{\DocumentationTok}[1]{\textcolor[rgb]{0.73,0.13,0.13}{\textit{{#1}}}}
    \newcommand{\AnnotationTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    \newcommand{\CommentVarTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    \newcommand{\VariableTok}[1]{\textcolor[rgb]{0.10,0.09,0.49}{{#1}}}
    \newcommand{\ControlFlowTok}[1]{\textcolor[rgb]{0.00,0.44,0.13}{\textbf{{#1}}}}
    \newcommand{\OperatorTok}[1]{\textcolor[rgb]{0.40,0.40,0.40}{{#1}}}
    \newcommand{\BuiltInTok}[1]{{#1}}
    \newcommand{\ExtensionTok}[1]{{#1}}
    \newcommand{\PreprocessorTok}[1]{\textcolor[rgb]{0.74,0.48,0.00}{{#1}}}
    \newcommand{\AttributeTok}[1]{\textcolor[rgb]{0.49,0.56,0.16}{{#1}}}
    \newcommand{\InformationTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    \newcommand{\WarningTok}[1]{\textcolor[rgb]{0.38,0.63,0.69}{\textbf{\textit{{#1}}}}}
    
    
    % Define a nice break command that doesn't care if a line doesn't already
    % exist.
    \def\br{\hspace*{\fill} \\* }
    % Math Jax compatibility definitions
    \def\gt{>}
    \def\lt{<}
    \let\Oldtex\TeX
    \let\Oldlatex\LaTeX
    \renewcommand{\TeX}{\textrm{\Oldtex}}
    \renewcommand{\LaTeX}{\textrm{\Oldlatex}}
    % Document parameters
    % Document title
    \title{Appendix: Codes of the Examples}
    \date{\vspace{-5ex}}
    
    
    
% Pygments definitions
\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@fm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vm\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sa\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@dl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother


    % For linebreaks inside Verbatim environment from package fancyvrb. 
    \makeatletter
        \newbox\Wrappedcontinuationbox 
        \newbox\Wrappedvisiblespacebox 
        \newcommand*\Wrappedvisiblespace {\textcolor{red}{\textvisiblespace}} 
        \newcommand*\Wrappedcontinuationsymbol {\textcolor{red}{\llap{\tiny$\m@th\hookrightarrow$}}} 
        \newcommand*\Wrappedcontinuationindent {3ex } 
        \newcommand*\Wrappedafterbreak {\kern\Wrappedcontinuationindent\copy\Wrappedcontinuationbox} 
        % Take advantage of the already applied Pygments mark-up to insert 
        % potential linebreaks for TeX processing. 
        %        {, <, #, %, $, ' and ": go to next line. 
        %        _, }, ^, &, >, - and ~: stay at end of broken line. 
        % Use of \textquotesingle for straight quote. 
        \newcommand*\Wrappedbreaksatspecials {% 
            \def\PYGZus{\discretionary{\char`\_}{\Wrappedafterbreak}{\char`\_}}% 
            \def\PYGZob{\discretionary{}{\Wrappedafterbreak\char`\{}{\char`\{}}% 
            \def\PYGZcb{\discretionary{\char`\}}{\Wrappedafterbreak}{\char`\}}}% 
            \def\PYGZca{\discretionary{\char`\^}{\Wrappedafterbreak}{\char`\^}}% 
            \def\PYGZam{\discretionary{\char`\&}{\Wrappedafterbreak}{\char`\&}}% 
            \def\PYGZlt{\discretionary{}{\Wrappedafterbreak\char`\<}{\char`\<}}% 
            \def\PYGZgt{\discretionary{\char`\>}{\Wrappedafterbreak}{\char`\>}}% 
            \def\PYGZsh{\discretionary{}{\Wrappedafterbreak\char`\#}{\char`\#}}% 
            \def\PYGZpc{\discretionary{}{\Wrappedafterbreak\char`\%}{\char`\%}}% 
            \def\PYGZdl{\discretionary{}{\Wrappedafterbreak\char`\$}{\char`\$}}% 
            \def\PYGZhy{\discretionary{\char`\-}{\Wrappedafterbreak}{\char`\-}}% 
            \def\PYGZsq{\discretionary{}{\Wrappedafterbreak\textquotesingle}{\textquotesingle}}% 
            \def\PYGZdq{\discretionary{}{\Wrappedafterbreak\char`\"}{\char`\"}}% 
            \def\PYGZti{\discretionary{\char`\~}{\Wrappedafterbreak}{\char`\~}}% 
        } 
        % Some characters . , ; ? ! / are not pygmentized. 
        % This macro makes them "active" and they will insert potential linebreaks 
        \newcommand*\Wrappedbreaksatpunct {% 
            \lccode`\~`\.\lowercase{\def~}{\discretionary{\hbox{\char`\.}}{\Wrappedafterbreak}{\hbox{\char`\.}}}% 
            \lccode`\~`\,\lowercase{\def~}{\discretionary{\hbox{\char`\,}}{\Wrappedafterbreak}{\hbox{\char`\,}}}% 
            \lccode`\~`\;\lowercase{\def~}{\discretionary{\hbox{\char`\;}}{\Wrappedafterbreak}{\hbox{\char`\;}}}% 
            \lccode`\~`\:\lowercase{\def~}{\discretionary{\hbox{\char`\:}}{\Wrappedafterbreak}{\hbox{\char`\:}}}% 
            \lccode`\~`\?\lowercase{\def~}{\discretionary{\hbox{\char`\?}}{\Wrappedafterbreak}{\hbox{\char`\?}}}% 
            \lccode`\~`\!\lowercase{\def~}{\discretionary{\hbox{\char`\!}}{\Wrappedafterbreak}{\hbox{\char`\!}}}% 
            \lccode`\~`\/\lowercase{\def~}{\discretionary{\hbox{\char`\/}}{\Wrappedafterbreak}{\hbox{\char`\/}}}% 
            \catcode`\.\active
            \catcode`\,\active 
            \catcode`\;\active
            \catcode`\:\active
            \catcode`\?\active
            \catcode`\!\active
            \catcode`\/\active 
            \lccode`\~`\~ 	
        }
    \makeatother

    \let\OriginalVerbatim=\Verbatim
    \makeatletter
    \renewcommand{\Verbatim}[1][1]{%
        %\parskip\z@skip
        \sbox\Wrappedcontinuationbox {\Wrappedcontinuationsymbol}%
        \sbox\Wrappedvisiblespacebox {\FV@SetupFont\Wrappedvisiblespace}%
        \def\FancyVerbFormatLine ##1{\hsize\linewidth
            \vtop{\raggedright\hyphenpenalty\z@\exhyphenpenalty\z@
                \doublehyphendemerits\z@\finalhyphendemerits\z@
                \strut ##1\strut}%
        }%
        % If the linebreak is at a space, the latter will be displayed as visible
        % space at end of first line, and a continuation symbol starts next line.
        % Stretch/shrink are however usually zero for typewriter font.
        \def\FV@Space {%
            \nobreak\hskip\z@ plus\fontdimen3\font minus\fontdimen4\font
            \discretionary{\copy\Wrappedvisiblespacebox}{\Wrappedafterbreak}
            {\kern\fontdimen2\font}%
        }%
        
        % Allow breaks at special characters using \PYG... macros.
        \Wrappedbreaksatspecials
        % Breaks at punctuation characters . , ; ? ! and / need catcode=\active 	
        \OriginalVerbatim[#1,codes*=\Wrappedbreaksatpunct]%
    }
    \makeatother

    % Exact colors from NB
    \definecolor{incolor}{HTML}{303F9F}
    \definecolor{outcolor}{HTML}{D84315}
    \definecolor{cellborder}{HTML}{CFCFCF}
    \definecolor{cellbackground}{HTML}{F7F7F7}
    
    % prompt
    \makeatletter
    \newcommand{\boxspacing}{\kern\kvtcb@left@rule\kern\kvtcb@boxsep}
    \makeatother
    \newcommand{\prompt}[4]{
        \ttfamily\llap{{\color{#2}[#3]:\hspace{3pt}#4}}\vspace{-\baselineskip}
    }

